The Random Conditional Distribution for Higher-Order Probabilistic Inference

The need to condition distributional properties such as expectation, variance, and entropy arises in algorithmic fairness, model simplification, robustness and many other areas. At face value however, distributional properties are not random variables, and hence conditioning them is a semantic error and type error in probabilistic programming languages. On the other hand, distributional properties are contingent on other variables in the model, change in value when we observe more information, and hence in a precise sense are random variables too. In order to capture the uncertain over distributional properties, we introduce a probability construct -- the random conditional distribution -- and incorporate it into a probabilistic programming language Omega. A random conditional distribution is a higher-order random variable whose realizations are themselves conditional random variables. In Omega we extend distributional properties of random variables to random conditional distributions, such that for example while the expectation a real valued random variable is a real value, the expectation of a random conditional distribution is a distribution over expectations. As a consequence, it requires minimal syntax to encode inference problems over distributional properties, which so far have evaded treatment within probabilistic programming systems and probabilistic modeling in general. We demonstrate our approach case studies in algorithmic fairness and robustness.

==> content.tex <==
\graphicspath{{figures/}}


% \subsection{snippets}
% Many image processing problems can be formalized as the recovery of an
% image $f \in \mathbb{R}^n$ from a set of $p \leq n$ noisy linear measurements:

% $$
% y = \phi f + \epsilon \in \mathbb{R}
% $$

% Ok so a few things; most methods talk about noise, because we can't observe our data exactly.
% Most methods use a linear operator.
% everyone uses the term ill-posed; I should use that..
% Big focus on linear inverse problems:

% linear inverse problems frequently lead to integral
% equations of the first kind, which is why such equations play an important

% many inverse problems are inherently nonlinear even if the corresponding direct problem is linear.

% When using the term inverse problem, one immediately is tempted to ask "inverse
% to what?". Following J.B. Keller [150], one calls two problems inverse to each other
% if the formulation of one problem involves the other one. For mostly historic reasons,
% one might call one of these problems (usually the simpler one or the one which was
% studied earlier) the direct problem, the other one the inverse problem. However,
% if there is a real-world problem behind the mathematical problem studied, there
% is, in most cases, a quite natural distinction between the direct and the inverse
% problem. E.g., if one wants to predict the future behaviour of a physical system
% from knowledge of its present state and the physical laws (including concrete values
% of all relevant physical parameters), one will call this the direct problem. Possible
% inverse problems are the determination of the present state of the system from future
% observations (i.e., the calculation of the evolution of the system backwards in time)
% or the identification of physical parameters from observations of the evolution of the
% system (parameter identification).
% There are, from the applications point of view, two different motivations for 
% studying such inverse problems: first, one wants to know past states or parameters of a
% physical system. Second, one wants to find out how to influence a system via its
% present state or via parameters in order to steer it to a desired state in the future.

% As we will see, such inverse problems most often do not fulfill Hadamard's 
% postulates of well-posedness (see Chapter 2). They might not have a solution in the
% strict sense, solutions might not be unique and/or might not depend continuously
% on the data. Mathematical problems having these undesirable properties are called
% ill-posed problems (improperly posed problems) and pose (mostly because of the 
% discontinuous dependence of solutions on the data) severe numerical difficulties. While
% the study of concrete inverse problems frequently involves the question how to 
%   uniqueness by additional information or assumptions, not much can be said
% about this in a general context. The aspect of lack of stability and its restoration by
% appropriate methods (regularization methods), however, can be treated in sufficient
% generality. The theory of regularization methods is well-developed for linear inverse
% problems and at least emerging for nonlinear problems and forms the core of this


\section{Introduction}
Problems in vision, robotics, statistical inference and many examples in the natural sciences are naturally posed as inverse problems.
Often we can simulate a model in the forward (typically causal) direction, but the inverse direction is ill-posed. For instance, current computer graphics techniques can render realistic images from a given 3D environment but the inverse problem of inferring geometry, lighting, viewpoint, etc. from an image is a non trivial problem of vision.
Probability theory and regularized optimization have been used extensively to formalize inverse problems, but algorithms based on these principles typically use the forward program as a black-box, ignore its structure, and perform poorly when the domain is highly structured or solutions are very sparse.
In contrast, the programming languages community has 
explored program inversion in the context of program synthesis~\cite{srivastava2011path}, but these systems either assume that the function is invertible, or they enumerate all possible inputs that map to the target output, rendering them inapplicable to problems in the aforementioned domains.
We present the first approach to program inversion that both exploits program structure and is applicable to programs which may be non-injective, non-linear, or map between high dimensional or highly constrained spaces.

% Computing a function from output to input is often dramatically more challenging than from input to output.
% % For a given causal process that we can simulate, the corresponding inverse process is often an inference problem important to artificial intelligence.
% % This presents a challenge, because many of the most important problems in artificial intelligence can be framed as an inverse simulation of a model.
% Modern computer graphics, for example, can simulate billions of light rays interacting with complex geometry and materials to render images that are indistinguishable from reality.
% In contrast, the inverse problem of inferring geometry, lighting, viewpoint and surface material from an image remains a distant dream of computer vision.
% % This gap appears time and time again - in inverse kinematics, inverse planning, inverse optimal control, and in various inverse problems found in the natural sciences and engineering.
% That this gap appears time and time again across many domains is at odds with an observation that spurred this contribution: the composition of a program dictates, at least in part, a program to compute an inverse.

% \rework{end of first paragraph:by using program structure/PL techniques can dramatically simplify problem of inversion}

\subsection{Problem formulation}
The inverse problem for non-invertible functions is commonly posed as a constrained optimization problem.
Since the forward process $f$ loses information by collapsing several inputs $x$ to the same output $y$, the inverse process from $y$ to $x$ is ambiguous.
A loss term $\mathcal{L}(x)$ enforces uniqueness: $\mathcal{L}$ is chosen such that of the multiple $x$ that $f$ maps to a $y$, $\argmin_x \mathcal{L}(x)$ is unique and maximizes a desired property.
Given $y$, we then seek $x^*$:
\begin{equation}\label{eq:inverseproblem}
x^* = \argmin_x \mathcal{L}(x) \ \textrm{ where } \ f(x) = y
\end{equation}

% This framework is inefficient in the long run, because each new element $y \in Y$ requires a new optimization process.
% To remedy this, problems which demand rapid inversion of many inputs have been cast as inverse mapping problems.
% Rather than find each x separately, an inverse mapping is a function $h(y) = x$ that can be quickly deployed on new inputs.
% $h$ is optimal if it minimizes $\mathcal{L}$ over a set of inputs $Y$:
% \begin{equation}\label{eq:inversemap}
% h^* = \argmin_h \sum_{y \in Y} \mathcal{L}(h(y), y) \ \textrm{ where } \ f(h(y)) = y
% \end{equation}
Different kinds of problem can be formulated in these terms.
In inference problems such as the aforementioned example in vision, $f$ models a process that constructs observable values from unobserved causes;
$\mathcal{L}$ should then be designed to favor the most probable cause of given observations.
In control problems such as inverse kinematics, $f$ maps variables under control (e.g. the joint angles of a robot) to variables we wish to control (the position of the hand); 
$\mathcal{L}$ should encode any additional desiderata (e.g. to minimize energy consumption or torques applied to the motors).
% $\mathcal{L}$ may also be a generic measure, promoting sparsity \cite{}, robustness, or simplicity for example.

Formulation \ref{eq:inverseproblem} is often intractable to apply directly because the constraint $f(x) = y$ demands we invert $f$, which may be complex and nonlinear, or map between spaces which are highly-constrained or high-dimensional.
Finding \emph{any} solution, let alone the optimal solution, is often beyond the capabilities of exact constraint solvers.
A common workaround is to first construct a distance $d$ where $d(y_1,y_2)=0$ iff $y_1 = y_2$, then
add $d(f(x), y)$ as an optimality criteria so the entire problem can be solved with an unconstrained optimization algorithm. Unfortunately, when solutions are very sparse, minimizing a distance is no more tractable than solving the constraint.

\subsection{Parametric Inversion with Ali\=o}

In this paper, we present a system called Ali\=o that takes a very different approach to this problem. 
Rather than search over $x$ using $f$ to check consistency with $y$, Ali\=o starts with $y$ and literally computes $f$ in reverse, using our new theory of \emph{parametric inversion} to address the non-invertibility of $f$.

Parametric inversion generalizes function inversion to non-injective functions.
By definition, a non-invertible function $f$ maps multiple points to the same value, which implies a choice in the inverse direction: which $x$ should an inverse of $f$ map $y$ to?
If the number of choices is very large or even infinite, it becomes untenable to represent them explicitly.

A parametric inverse $f^{-1}(y; \theta)$ parameterizes this choice instead.
$f^{-1}$ is a parameterized function which maps an element $y$ to a single element of its preimage:
% By varying a parameter $\theta$, we vary over the values in the preimage of $y$:
\begin{equation}\label{eq:preimage}
f^{-1}(y; \theta) \in \{x \mid f(x) = y \}
\end{equation}
% $f^{-1}$ is
For example, while $f(x) = x^2$ is not invertible, we can define a parameter $\theta \in \{-1,1\}$ and parametric inverse $f^{-1}(y; \theta)  = \theta  \sqrt{y}$.
The parameter choice $\theta$ determines which element of the preimage $\{-\sqrt{y}, +\sqrt{y}\}$ is the output of $f^{-1}$.

For simple functions, it is generally easy to define parametric inverses by hand; the real power of our techniques comes from the ability to compute parametric inverses of function compositions in terms of the parametric inverses of the components, akin to the way the chain rule is used to compute derivatives from compositions of simple functions. This makes it possible for Ali\=o to automatically generate parametric inverses of programs represented as dataflow graphs.

We use parametric inverses to tackle the inverse problem \eqref{eq:inverseproblem}.
Rather than search over $X$, we search over $\Theta$:
\begin{equation}\label{eq:optinvtotal}
\theta^* = \argmin_\theta \mathcal{L}(f^{-1}(y; \theta))
\end{equation}
then:
\begin{equation}
x^* = f^{-1}(y; \theta^*)
\end{equation}

For any $x$ that is the output of a $f^{-1}$, the constraint $f(x) = y$ in \eqref{eq:inverseproblem} holds by definition of a parametric inverse, and the constrained optimization problem appears unconstrained.

There is one major complication with this approach. Given two parametric inverses $f_1^{-1}(y;\theta_1)$ and $f_2^{-1}(y; \theta_2)$, even if we know the domains $\Theta_1$ and $\Theta_2$ of $\theta_1$ and $\theta_2$, it is not always possible to compute a clean representation of the domain of the parameter for the composition. In fact, for some compositions, $f_1^{-1}\circ f_2^{-1}(y, \theta_{1,2})$, the domain of valid parameters $\theta_{1,2}$ may be a function of $y$ itself. This leads to an important empirical question of whether in practice it is easier to solve \eqref{eq:optinvtotal} compared to \eqref{eq:inverseproblem}, which we answer by evaluating the approach on problems from inverse kinematics and inverse graphics. 

In summary, our contribution is a foundational approach to both function and program inversion. The theory is realized in the Ali\=o framework, which is implemented as an embedded DSL in the Julia programming language \cite{Bezanson2012}. 
In more detail:

% \rework{What precisely are we going to give, (pi a y is going to search for best x*. And what can we show formally,) .}
% \todo{Make clear both foundational system and fully fledged working system}
% \todo{Have both case studies, and microbenchmarks}
\begin{itemize}
\item We introduce parametric inversion (Section \ref{parametric-inverses}) and discover properties that are critical for a parametric inverse to be useful in practice.
We manually define parametric inverses with these properties for several primitive functions (see table \ref{tab:inverses}).
\item We present a rule to construct a parametric inverse from a composition of primitives (Section \ref{parametric-inversion-of-composite-functions}), and prove that soundness and completeness of primitive inverses is preserved in the composition.
\item Totality is however not preserved by the composition rule. We root out the cause and develop two methods in response (Section \ref{partiality}).
\item We introduce Ali\=o dataflow (Section \ref{alio}) and extend parametric inversion to Ali\=o programs(Section \ref{invertalio}).
\end{itemize}

To evaluate our contribution we first use a number of micro-benchmarks to understand the advantages and limitations of parametric inversion (Section \ref{microanalysis}). Finally, we invert realistic problems from inverse kinematics and inverse graphics, and compare against optimization over the input (Section \ref{evaluation}).
First, supported by an example in inverse kinematics, we give a brief outline of the problem, our approach, and the main challenges that we must address.

\section{Inverse Kinematics Example}
In inverse kinematics, central to both robotics and computer animation, we seek joint angles which will drive a robot into the desired position.
The robot arm in figure \ref{fig:robotarm} can be modeled as a linkage system with links of length $1$ and the forward kinematic function which maps joint angles to Cartesian coordinates is then easily derived as $f(\varphi_{1,2,3}) = (x, y)$ where:
\begin{align}
x = \cos(\varphi_1) + \cos(\varphi_1 + \varphi_2) + \cos(\varphi_1 + \varphi_2 + \varphi_3) \label{fwdx} \\ 
y = \sin(\varphi_1) + \sin(\varphi_1 + \varphi_2) + \sin(\varphi_1 + \varphi_2 + \varphi_3) \label{fwdy}
\end{align}
For (almost all) target coordinates $x, y$, there are infinitely many solutions.
In robotics it is common to prefer solutions which minimize energy demands of the robot or torques applied to the motors for example.  In this case we prioritize small angles and minimize their absolute value:
$$
\mathcal{L}(\varphi_{1,2,3}) = |\varphi_1|+ |\varphi_2| + |\varphi_2|
$$
The standard approach is then to use optimization.

% (\varphi_1, \varphi_2, \varphi_3)* = \argmin_x d(f(\varphi_1, \varphi_2, \varphi_3), (x,y)) + \mathcal{L}(\varphi_1, \varphi_2, \varphi_3)
% \end{equation}

\begin{equation}\label{eq:inversekinematics}
\varphi^*_{1,2,3} = \argmin_{\varphi_{1,2,3}} d(f(\varphi_{1,2,3}), (x,y)) + \mathcal{L}(\varphi_{1,2,3})
\end{equation}

\begin{figure}[!htb]
\centering
\includegraphics[width=0.5\linewidth]{ik}
\caption{Robot linkage arm}
\label{fig:robotarm}
\end{figure}

% \begin{lstlisting}
% """
% function f(φ1, φ2, φ1)
%   x = sin(\varphi 1) + sin(φ1, φ2) + sin(φ1, φ2, φ3)
%   y = sin(φ1) + sin(φ1, φ2) + sin(φ1, φ2, φ3)
%   return (x, y)
% end

% invf = inv(f)
% \end{lstlisting}

As the name suggests, inverse kinematics requires inverting $f$; the optimization in \eqref{eq:inverseproblem} achieves this implicitly by executing the forward function many times and aiming to find angles $\varphi_{1, 2, 3}$ that map to the given coordinates $(x, y)$.

Conceptually, rather than guess values of $\varphi_{1, 2, 3}$ and check whether the constraints are satisfied, a parametric inverse starts with the constraints and works backwards. Given $(x, y)$ the goal is to find a parametric representation of possible $\varphi_{1, 2, 3}$ values. Considering each of \eqref{fwdx} and \eqref{fwdy} separately let us manually construct a parametric inverse of $f(\varphi_{1, 2, 3}) = (x, y)$. Using two parameters for each equation we obtain the three elements that sum up to $x, y$ respectively
\begin{equation*}
\cos(\varphi_1) = x - \theta^x_1 - \theta^x_2, \cos(\varphi_1+\varphi_2) = \theta^x_1, \cos(\varphi_1+\varphi_2+\varphi_3) = \theta^x_2
\end{equation*}
\begin{equation*}
\sin(\varphi_1) = y - \theta^y_1 - \theta^y_2, \sin(\varphi_1+\varphi_2) = \theta^y_1, \sin(\varphi_1+\varphi_2+\varphi_3) = \theta^y_2
\end{equation*}

Since $\mathcal{L}(\varphi_{1, 2, 3})$ prioritizes small angles and for the sake of simplicity, assume $\varphi_{1, 2, 3}$ to be small enough such that $\arcsin$, $\arccos$ are used as inverses of $\sin, \cos$:
\begin{align}
\varphi_1 = \arccos(x - \theta_1^x - \theta_2^y) = \arcsin(y - \theta_1^y - \theta_2^y) \label{constrain1} \\
\varphi_2 = \arccos{\theta_1^x} - \varphi_1 = \arcsin{\theta_1^y} - \varphi_2 \label{constrain2} \\
\varphi_3 = \arccos{\theta_2^x} - \varphi_1 - \varphi_2 = \arcsin{\theta_2^y} - \varphi_1 - \varphi_2 \label{constrain3}
\end{align}

The equations above together constitute a parametric inverse $f^{-1}(x, y; \theta)$ of $f$ that can be used in solving \eqref{eq:inversekinematics} by looking for the optimal value of $\theta = (\theta_1^x, \theta_2^x, \theta_1^y, \theta_2^y)$ instead.

\begin{equation}
\theta^* = \argmin_{\theta \in \mathbb{R}^4} \mathcal{L}(f^{-1}(x, y; \theta))
\end{equation}

Handling the inversion constraint with $d(f(\varphi_{1, 2, 3}), (x, y))$ in \eqref{eq:inversekinematics} is no longer a concern.
However, notice that
%due to the reuse of values in \eqref{fwdx}, \eqref{fwdy} when computing $f$ 
the resulting equations \eqref{constrain1}, \eqref{constrain2}, \eqref{constrain3} put constraints on the possible values of $\theta$ that would yield a valid $\varphi_{1, 2, 3}$. We address this issue and show that both optimization and symbolic reasoning can be used to solve it.

% First, although not critical, it is more convenient to represent the forward kinematic function as a dataflow process.
% \rework{Finish example}

% %\todo{not mentioned in text}
% \begin{figure}[!htb]
% \centering
% \includegraphics[width=0.75\linewidth]{flowrobo1.png}
% \includegraphics[width=0.75\linewidth]{flowrobo2.png}
% \caption{Forward kinematic function given by \eqref{fwdx} and \eqref{fwdy} and its parametric inverse - Inverse kinematic}
% \end{figure}\label{flowrobo}

\section{Parametric Inversion}\label{parametric-inverses} 

Parametric inversion generalizes function inversion to non-invertible functions.
A parametric inverse is a parameterized function which maps an element $y$ to a single element of its preimage (figure \ref{fig:pi}):
% The parameter choice $\theta$ determines which element of the preimage, $f^{-1}$ outputs.
\begin{definition}A function $f^{-1} : Y \times \Theta \to X$ is a sound parametric inverse of $f: X \to Y$ if for all $y$ in the image of $f$, for all $\theta \in \Theta$:
\begin{equation}\label{eq:pinv}
f^{-1}(y; \theta) \in  \{x \mid f(x) = y \}\end{equation}\end{definition}

In contrast to a conventional inverse, a parametric inverse always exists.
For example, while $f(x) = x^2$ is not invertible, we can define a parameter space $\theta \in \{-1,1\}$ and parametric inverse $f^{-1}(y; \theta)  = \theta \sqrt{y}$.
The parameter choice $\theta$ determines which element of the preimage $\{-\sqrt{y}, +\sqrt{y}\}$ is output.
$f^{-1}$ exists even if $f$ is injective; $f^{-1}(y;\theta)$ is then the single member of the preimage of $y$, regardless of $\theta$.

If a function takes multiple inputs, its parametric inverse will return a tuple.
For example, inverse addition (denote $+^{-1}$) maps a value $y$ to two values whose sum is $y$: $+^{-1}(y; \theta) = (y - \theta, \theta)$, where $\theta \in \mathbb{R}$.
Parametric inverses are not unique; it is equally valid to define $+^{-1}(y; \theta) = (-\theta, y + \theta)$.

A parametric inverse is most useful when it can recover any element of the preimage of any $y$, i.e., it is \textit{complete}:
\begin{definition}\label{def:complete}
$f^{-1}$ is a complete parametric inverse of $f$ if for all $y$, for all $x \in \{x \mid f(x)  = y\}$, there exists $\theta$ such that $f^{-1}(y; \theta) = x$.
\end{definition}
Inverse addition as $+^{-1}(y; \theta) = (0, y)$ is sound but not complete; there exists no $\theta$ such that for instance $+^{-1}(0;\theta) = (-2, 2)$, despite the fact that $-2 + 2 = 0$.
$+^{-1}(y; \theta_1, \theta_2) = (\theta_1, \theta_2)$ is complete but not sound; any pair of numbers that sum to $y$ can be recovered by an appropriate choice of $\theta_1, \theta_2$, but there are many more output pairs that do not sum to $y$. Several sound and complete parametric inverses of primitive functions are provided in Table \ref{tab:inverses}.
%, see supplementary information for a more comprehensive list.


\begin{figure}[!htb]
\centering
\includegraphics[width=0.95\linewidth]{fgraph}
\caption{A non-injective function $f$ (left) is non-invertible because it maps both $x_1$ and $x_2$ to $y$.  A parametric inverse $f^{-1}$ (right) uses a parameter $\theta$ to disambiguate between $x_1$ and $x_2$.}\label{fig:pi}
\end{figure}

\newcommand{\select}[2]{[#1]^{#2}}


\begin{table*}[h]%\label{tab:pinverses}
  \centering
  \begin{tabular}{ l | c | c | r }
  	$f$ & $X$ & $\Theta$ & $f^{-1}$ \\
    \hline
$x_1+x_2$ & $\mathbb{R}, \mathbb{R}$ & $\mathbb{R}$ & $y - \theta, \theta$ \\
$x_1-x_2$ & $\mathbb{R}, \mathbb{R}$ & $\mathbb{R}$ & $y + \theta, \theta$ \\
$x_1\cdot x_2$ & $\mathbb{R}, \mathbb{R}$ & $\mathbb{R} \setminus 0 \times \{0, 1\}$ & $\select{y/\theta_1, \theta_1}{\theta_2}, \select{\theta_1, y/\theta_1}{\theta_2}$ \\
$x_1 / x_2$ & $\mathbb{R}, \mathbb{R} \setminus 0$ & $\mathbb{R} \setminus 0$ & $y\cdot\theta, \theta$ \\
$x_1^{x_2}$ & $\mathbb{R}_{>0}, \mathbb{R}$ & $\mathbb{R} \setminus 0 \times \{0, 1\} \times \mathbb{R}$ & $\select{\theta_{1}, 1}{(1-y) \lor \theta_{2}}, \select{\log_{\theta_{1}}(y), \theta_{3}}{(1-y) \lor \theta_{2}}$ \\
$\log_{x_1}(x_2)$ & $\mathbb{R}_{>0}, \mathbb{R}_{>0} \setminus 1$ & $\mathbb{R}_{>0} \setminus 1$ & $\theta, \theta^y$ \\
% $x^n$ & $\mathbb{N}, \{-1, 1\}$ & $\theta_{2}z^{1/\theta_{1}}, \theta_{1}$ \\
$\abs(x)$ & $\mathbb{R}$ & $\{-1,1\}$ & $\theta \cdot y$ \\
$\min(x_1, x_2)$ & $\mathbb{R}, \mathbb{R}$ & $\mathbb{R}_{\geq 0} \times \{0, 1\}$ & $\select{y, y + \theta_1}{\theta_2}, \select{y + \theta_1, y}{\theta_2}$ \\
$\max(x_1, x_2)$ & $\mathbb{R}, \mathbb{R}$ & $\mathbb{R}_{\geq 0} \times \{0, 1\}$ & $\select{y, y - \theta_1}{\theta_2}, \select{y - \theta_1, y}{\theta_2}$ \\
$\cos(x)$ & $\mathbb{R}$ & $\mathbb{Z}$ & $2 \pi \lceil \frac{\theta}{2} \rceil + (-1)^{\theta} \arccos(y)$ \\
$\sin(x)$ & $\mathbb{R}$ & $\mathbb{Z}$ & $\pi \theta + (-1)^{\theta} \arcsin(y)$ \\
$\tan(x)$ & $\mathbb{R}$ & $\mathbb{Z}$ & $\pi \theta + \arctan(y)$ \\
% $cot(y)$ & $\mathbb{R}$ & $\mathbb{Z}$ & $\pi \theta + arccot(y)$ \\
$x_1 > x_2$ & $\mathbb{R}, \mathbb{R}$ & $\mathbb{R} \times \mathbb{R}_{>0}$ & $\theta_1, \select{\theta_1 - \theta_2, \theta_1 + \theta_2}{y}$ \\
$x_1 < x_2$ & $\mathbb{R}, \mathbb{R}$ & $\mathbb{R} \times \mathbb{R}_{>0}$ & $\theta_1, \select{\theta_1 + \theta_2, \theta_1 - \theta_2}{y}$\\
$x_1 = x_2$ & $\mathbb{R}, \mathbb{R}$ & $\mathbb{R} \times \mathbb{R} \setminus 0$ & $\theta_1, \select{\theta_1, \theta_1 + \theta_2}{y}$\\
$x_1 \land x_2$ & $\{0, 1\}, \{0, 1\}$ & $\{0, 1\} \times \{0, 1\}$ & $\select{y, \theta_{1} \land \theta_{2}}{y}, \select{y, \theta_{1} \oplus \theta_{2}}{y}$ \\
$x_1 \lor x_2$ & $\{0, 1\}, \{0, 1\}$ & $\{0, 1\} \times \{0, 1\}$ & $\select{\theta_{1} \lor \neg \theta_{2}, y}{y}, \select{\theta_{1} \oplus \theta_{2}, y}{y}$ FIXME WRONG!!!!!!!\\
$x_1 \oplus x_2$ & $\{0, 1\}, \{0, 1\}$ & $\{0, 1\} \times \{0, 1\}$ & $\theta_{1}, \theta_{1} \oplus y$ \\
    \hline
  \end{tabular}
\medskip
	  \caption{Primitive parametric inverses.  Column $f$ contains forward non-injective functions. The input space for the forward function $f$ is $X$ while $\Theta$ is the parameter space used for parametric inverses shown in column $f^{-1}$. $\select{a,b}{c}$ denotes if $c$ then $a$ else $b$, or $ac + b(1-c)$}\label{tab:inverses}
\end{table*}

% \begin{table}[h]%\label{tab:pinverses}
%   \centering
%   \resizebox{\linewidth}{!}{%
%   \begin{tabular}{ l | c | c | r }
%   	$f$ & $X$ & $\Theta$ & $f^{-1}$ \\
%     \hline
% $x_1+x_2$ & $\mathbb{R} \times \mathbb{R}$ & $\mathbb{R}$ & $y - \theta, \theta$ \\
% $x_1-x_2$ & $\mathbb{R}\times \mathbb{R}$ & $\mathbb{R}$ & $y + \theta, \theta$ \\
% $x_1\cdot x_2$ & $\mathbb{R} \times \mathbb{R}$ & $\mathbb{R} \setminus 0 \times \{0, 1\}$ & $\select{y/\theta_1, \theta_1}{\theta_2}, \select{\theta_1, y/\theta_1}{\theta_2}$ \\
% $x_1 / x_2$ & $\mathbb{R} \times \mathbb{R} \setminus 0$ & $\mathbb{R} \setminus 0$ & $y\cdot\theta, \theta$ \\
% $x^2$ & $\mathbb{R}$ & $\{-1, 1\}$ & $\theta \sqrt{y}$ \\

%     \hline
%   \end{tabular}
%   }
% \medskip
% 	  \caption{Primitive parametric inverses.  Column $f$ contains forward non-injective functions. The input space for the forward function $f$ is $X$ while $\Theta$ is the parameter space used for parametric inverses shown in column $f^{-1}$. $\select{a,b}{c}$ denotes if $c$ then $a$ else $b$, or $ac + b(1-c)$.}\label{tab:pinverses}
% \end{table}
% \begin{definition}A function $f^{-1} : Y \times \Theta \to X$ is a sound parametric inverse of $f: X \to Y$ if for all $\theta$:
% \begin{equation}\label{right-inverse}
% f(h(y)) = y \text{   where   } h(y) = f^{-1}(y; \theta)
% \end{equation}\end{definition}

% Fixing $\theta$ induces a right inverse $h$, 
% Condition \ref{right-inverse} is equivalent to condition \ref{eq:pinv}, but while previously each $\theta \in \Theta$ represented an element of the preimage of any $y$; here it represents a right-inverse of $f$.

\section{Parametric Inverses of Compositions}\label{parametric-inversion-of-composite-functions}

In this section we derive sound and complete parametric inverses of compositions of primitive functions, by reverse composition of parametric inverses of each primitive.
In section \ref{invertalio} we describe parametric inversion of programs in our language Ali\=o, but for both clarity and generality (parametric inversion is applicable to any kind of functional program) we present the mathematical foundations in terms of function compositions first.
% Our method is a generalization of the composition rule for invertible functions:
% If $f_1$ and $f_2$ are invertible, and $f=f_1 \circ f_2$, then $f^{-1}(z) = f^{-1}_2(f^{-1}_1(z))$.

% Let $f=f_1 \circ f_2$ be a composition where $f_1: X_1 \to Y_1$, $f_2: X_2 \to Y_2$ \todo{Will I lose anything by removing the types here} and $Y_2 \cap X_1 \neq \emptyset$.
% To construct a parametric inverse  $f^{-1}:Y_1 \times \Theta \to X_2$ we substitute $f_1$ and $f_2$ with their corresponding parametric inverses $f^{-1}_1$ and $f^{-1}_2$, and reverse the order of composition:
\begin{algowizm}
\label{algo:compinversion}
Let $f=f_1 \circ f_2$ be a composition.
To construct a parametric inverse $f^{-1}$, substitute $f_1$ and $f_2$ with their corresponding parametric inverses $f^{-1}_1$ and $f^{-1}_2$, reverse the order of composition, and concatenate the parameter spaces:
\begin{equation}\label{eq:compoverload}
f^{-1}(y;\theta_1, \theta_2) = f^{-1}_2(f^{-1}_1(y;\theta_1), \theta_2)
\end{equation}
The parameter space of $f^{-1}$ is $\Theta = \Theta_1 \times \Theta_2$, where $\Theta_i$ is the parameter space of primitive $f^{-1}_i$.
\end{algowizm}

For example, expressing $f(x) = x^4$ as $f = \sqr_1 \circ \sqr_2$ (where $\sqr(x) = x^2$), its parametric inverse $f^{-1}$ is then:
$$
f^{-1}(y; \theta_1, \theta_2) = \sqr_2^{-1}(\sqr_1^{-1}(y;\theta_1); \theta_2) = \theta_2\sqrt{\theta_1\sqrt{y}}
$$
We overload the composition operator $\circ$ to denote composition of domains and concatenation of parameter spaces. That is, $f^{-1} = f^{-1}_2 \circ f^{-1}_1$ denotes that $f^{-1}$ is defined as in equation \eqref{eq:compoverload}.
With this notation the parametric inversion composition rule exactly mirrors the well-known inverse composition rule of invertible functions \cite{lay2006}:
\begin{equation}
(f_1\circ f_2)^{-1} = f_2^{-1}\circ f_1^{-1}
\end{equation}
\begin{theorem}
\label{thm:soundcomplete}
$f^{-1}$ is a sound and complete parametric inverse of $f$.

\textit{Proof.}
See supplementary information.

\end{theorem}



\section{The Curse of Partiality}\label{partiality}

The inverse composition rule \eqref{eq:compoverload} generalizes naturally to arbitrary programs (Section \ref{alio}); yet parametric inversion is not trivial.
The problem is that $f^{-1}$ will often be undefined on a large portion of the parameter space that the algorithm constructs it on: $\Theta = \Theta_1 \times \Theta_2$.
% and the constrained optimization problem over $X$ can be tackled instead as an optimization over $\Theta$:
% \begin{equation}
% \theta^* = \argmin_\theta \mathcal{L}(f^{-1}(y; \theta))
% \end{equation}
% $x^*$ is then simply:
% \begin{equation}
% x^* = f^{-1}(y; \theta^*)
% \end{equation}
The previous example $f^{-1}(y; \theta_1, \theta2) = \theta_2\sqrt{\theta_1\sqrt{y}}$ is undefined when $\theta_1 = -1$, regardless of $y$, and hence is a partial function with respect to its parameter space; or simply a partial parametric inverse:

% Table \ref{tab:inverses} contains examples of parametric inverses which are sound, complete and also \textit{total}:

\begin{definition}A parametric inverse $f^{-1}$ is partial if there exists some $\theta$ and some $y$ in the image of $f$ such that $f^{-1}(y; \theta) = \bot$, where $\bot$ (read as "bottom") means undefined.
A parametric inverse is total if it is not partial.
\end{definition}

% Parametric inverse multiplication $\times^{-1}(z; \theta) = (z / \theta, \theta)$ is partial if $\Theta=\mathbb{R}$, since it is undefined at $\theta = 0$, but total if $\Theta=\mathbb{R} \setminus 0$.
% Partiality refers to the product $Y \times \Theta$ and not only $Y$.
% Note that this $\times^{-1}$ is also not complete (when $z = 0$); table \ref{tab:inverses} contains a more complex, complete inverse.

% \begin{definition}
% A partial parametric inverse $f^{-1}$ is sound, if for all $y$ and $\theta$, when $f^{-1}(y; \theta)$ is defined, $f^{-1}$ satisfies equation \eqref{eq:pinv}.
% \end{definition}

% Each inverse primitive $f^{-1}_i$ parameterizes different ways to undo the corresponding forward primitive $f_i$; if it permits more scenarios than could possibly occur in the forward computation.
The problem that partiality causes is not fully captured by its definition, nor resolved by simply redefining a parametric inverse onto the constrained parameter space upon which it is total.
If it is just as challenging to find $\theta$ which satisfies $f^{-1}(y; \theta) \neq \bot$ as it is to find $x$ which satisfies $f(x) = y$, parametric inversion has limited utility.
In other words, for a parametric inverse to be useful it should be total with respect to a parameter space which is easy to select points from.
This criteria is subjective to a degree, but in practice we mean parameter spaces which are unconstrained such as $\mathbb{R}$ or $\mathbb{N}$, bounded or unbounded intervals, sets that can be efficiently stored explicitly such as $\{-1, 1\}$, and combinations thereof.
% Compounding this, partiality presents an obstacle to optimization because if $f^{-1}$ is partial, we unable to compute a loss i.e. $\mathcal{L}(f^{-1}(y; \theta)) = \bot$.
% Partiality threatens any potential benefits of parametric inversion.

To address the problem of partiality we must first understand its cause, which rests upon subtle distinctions in the meaning of the domain of a function.
As is well known, the domain $X$ of a partial function $f:X \to Y$ is larger than $X'$ - the set of values it maps from (also referred to as its preimage).
A further distinction arises when considering $f$ as an element of a composition $\cdots \circ d \circ e \circ f \circ g \circ h \circ \cdots$.
If the functions $g, h, \dots$ which precede $f$ restrict the set of possible inputs to $f$ \todo{Than would otherwise be the case}, then within the context of the composition the domain of $f$ is effectively reduced.
% $X'$ will then in turn be larger than the set of values $X''$ that are possible inputs to $f$.
We call the domain of a function within the context of a composition its \emph{effective domain}.

A parametric inverse constructed by algorithm \ref{algo:compinversion} is partial because the algorithm substitutes each primitive ignoring its context within the forward composition.
In particular, it replaces $f_i$ with an inverse that is complete with respect to the domain of $f_i$ and not the effective domain of $f_i$.
% Partiality occurs when for $f_1^{-1}$ in $f^{-1}$ there exists a parameter $\theta_1$ that maps to a value that is not in the domain of $f_2^{-1}$. 
For example, whenever $\theta_1 = -1$, the primitive $\sqr_1^{-1}$ in $\sqr_2^{-1} \circ \sqr_1^{-1}$ outputs a negative value, which is not in the domain of $\sqr_2^{-1}$.
This was inevitable because $\sqr_1^{-1}$ was constructed to be a complete parametric inverse of $\sqr_1$, ignoring that the effective domain of $\sqr_1$ in the forward composition $\sqr_1 \circ \sqr_2$ was limited to $\mathbb{R}^+$ by $\sqr_2$.
We visualize this in figure \ref{fig:partiality}, and in the supplementary information
provide a general formulation of when partiality occurs.
\begin{figure}[!htb]
\centering
\includegraphics[width=0.75\linewidth]{fgraph2}
\caption{The causes of partiality in composite parametric inverses. The composite forward function $f_1 \circ f_2$ (top) is total and surjective. However, its primitive $f_2$ is not surjective since it maps no value to $y_2$, which reduces the effective domain of $f_1$ from $\{y_1, y_2\}$ to $\{y_1\}$.  Algorithm \ref{algo:compinversion} constructs its parametric inverse (bottom) without this information, and substitutes to $f^{-1}_1$ complete with respect to the domain (and not effective domain) of $f_1$.  There must then exists a parameter ($\theta_2^b$) that maps to $y_2$; hence the inverse is partial.}\label{fig:partiality}
\end{figure}
Our running example can be turned into a total parametric inverse (totalized) manually, hinting at automated methods scribed in section \ref{unsoundtotal} and \ref{paramreduction}.
% To totalize a parametric inverse we must ensure that each possible output of every $f_i^{-1}$ in $f^{-1}$ is a possible input to $f_i$ in $f$. 
To make $(\sqr_1 \circ \sqr_2)^{-1}$ total, we observe that $\sqr_1^{-1}(y; \theta_1) = \theta_1\sqrt{y}$ is positive only if $\theta_1 = 1$, and hence fix $\theta_1 = 1$ to yield $\sqr^{-1}(\sqr^{-1}(y;1); \theta_2) = \theta_2\sqrt[4]{y}$.

\subsection{Totalization}\label{unsoundtotal}
Since our objective is to use a parametric inverse $f^{-1}$ for inverse problems \eqref{eq:inverseproblem}, we (temporarily) permit constraints on its parameter space to be violated.
From a sound but partial parametric inverse $f^{-1}$ we will derive an unsound parametric inverse $\apinv{f}$ which is (i) total, and (ii) consistent with $f^{-1}$,  i.e. $\apinv{f}(y; \theta) =  f^{-1}(y; \theta)$ when $f^{-1}(y; \theta) \neq \bot$.

A composite parametric inverse $f^{-1}$ derived from total primitives is partial if and only if $f_i^{-1}(y'; \theta_i) = \bot$ for at least one primitive $f_i$, where $y'$ is the output of the previous primitive in the composition or $y$ itself.
To make $f^{-1}$ total, it therefore suffices to totalize each primitive individually.
We introduce \emph{contraction} functions within the composition that funnel the flow of values to guarantee  that they are never outside the domain of any primitive.

\begin{definition}A contraction between $f:X \to Y$ and $g: Y' \to Z$ is a total function $c: Y \to Y'$ which contracts the codomain of $f$ to the domain of $g$. $c$ satisfies: 
\begin{equation}\label{eq:c}
c(y)=
\begin{cases}
    y & \text{if } y \in Y' \\
    \text{any } y' \in Y' & \text{otherwise }
\end{cases}
\end{equation}
\end{definition}

The following procedure totalizes  $f^{-1}$ by placing contractions between each pair of primitives:
\begin{algowizm}\label{algo:contraction}
Insert a contraction $c_i$ between each pair of primitives $f^{-1}_i$ and $f^{-1}_{i-1}$ to construct $f^{-1}_{i} \circ c_i \circ f^{-1}_{i-1}$.
$c_i$ restricts the codomain of $f^{-1}_{i-1}$ to the domain of $f^{-1}_{i}$:

\end{algowizm}
Since $\sqr_2^{-1} \circ \sqr_1^{-1}$ is undefined when the input to $\sqr^{-1}_2$ is negative, it can be totalized with a contraction that restricts $\mathbb{R}$ to $\mathbb{R}^+$.
$\sqr^{-1}_2 \circ \clip_{0,\infty} \circ \sqr_1^{-1}$ is an example of such totalization, where $\clip_{a,b}(x) = \max(a, \min(b, x))$ clips its input to the closest point in the interval $[a,b]$.
$\clip$ is not unique in satisfying \eqref{eq:c}.

$\apinv{f}$ is unsound but not arbitrarily so.
There is a subset of \todo{Not right, its Y cross Theta. Use same notation here as in constraint solving and explain the dependence of Y, i.e. why its not just subset of theta} $\Theta' \subset \Theta$ on which $\apinv{f}$ is both sound and complete.
This is crucial, because by completeness, for any $x^*$ that we seek there exists a corresponding $\theta^*$ which is both $\Theta'$ and $\Theta'$.
For some $\theta \in \Theta \setminus \Theta'$---the `bad' part of the parameter space-- unsound totalization makes it possible to compute a distance (and possibly direction) to $\Theta'$ rather than simply $\bot$, and then use optimization to recover $\theta \in \Theta'$.

The degree to which constraints are violated can be efficiently measured in at least two ways.
\emph{identity loss} measures the extent to which the given inputs result in an element of the preimage.

\begin{definition}
The identity loss on (input, parameter) tuple $(y, \theta)$ is given by
\begin{equation}
\mathcal{L}_{id}(f; y, \theta) = d(f(f^{-1}(y; \theta)), y)
\end{equation}
\end{definition}

\emph{Domain loss} measures the distance between given inputs and the effective domain of each primitive.

\begin{definition}
The domain loss of a primitive $p : S \to V$ with $S_1$ effective domain is $\mathcal{L}_{dm}(p; s) = \inf_{s_1 \in S_1} d(s, s_1)$. The domain loss of a composite function $f = f_1 \circ ... \circ f_n$ is the sum of the domain losses of its primitives
\begin{equation}
\mathcal{L}_{dm}(f; x) = \sum_{i=1}^n \mathcal{L}_{dm}(f_i; x_i)
\end{equation}
\end{definition}

$\mathcal{L}_{id}$ of the forward function is zero when $\mathcal{L}_{dm}$ of the parametric inverse is zero but the reverse implication does not necessarily hold. The contractions from algorithm \ref{algo:contraction} allow $\mathcal{L}_{id} = 0$ even when having a pre-totalized parametric inverse with a nonzero $\mathcal{L}_{dm}$.
\begin{theorem}
If for a given $y \in Y, \theta \in \Theta$ the domain loss of $f^{-1}$ is $0$, then the identity loss of $f$ is also $0$:
\begin{equation}\label{dmid}
\mathcal{L}_{dm}(f^{-1}; y, \theta) = 0 \implies \mathcal{L}_{id}(f; y, \theta) = 0
\end{equation}

\textit{Proof.}
See supplementary information.

\end{theorem}

% Provided we can define a distance measure $d$ on $Y$, it is straightforward to compute a degree of soundness:
% $$
% \mathcal{L}^1_{\apinv{f}}(y) = d(f(\apinv{f}(y; \theta)),y)
% $$
% Alternatively, we can accumulate a more granular loss from every primitive in the composition.
% In $f^{-1}_{i} \circ c_i \circ f^{-1}_{i-1}$, let $Y_{i}$ be the domain of $f^{-1}_i$, then:
% $$
% \mathcal{L}^2_{\apinv{f}}(y; \theta) = \sum_i d(\apinv{f}_i(y_i; \theta_i), Y_{i+1})
% $$
% $d(y, Y)$ is the distance from $y$ to the closest point in $Y$, e.g. $d(y, [l, h])  = \max(y-u, l-y, 0)$.
% $\mathcal{L}^1$ is zero when $\mathcal{L}^2$ is zero but the reverse implication does not necessarily hold.
% In practice, they define loss surfaces with different optimization characteristics (figure  \ref{fig:diffloss}).
% $\mathcal{L}^2$ is useful if a meaningful distance on $Y$ does not exist.



% \section{Parametric Function Spaces}\label{fspaces}
% We can now attempt to construct an inverse mapping $h^*$ that is optimal with respect to $\mathcal{L}$.
% For any $\theta$ we can construct a candidate inverse mapping $h_\theta(y) = f^{-1}(y; \theta)$.
% $h_\theta$ is a right-inverse of $f$ since $f \circ h_\theta = \operatorname{id}$, i.e. composing $f$ with $h_\theta$ from the right gives the identity function.
% % $h_\theta$ solves the constraint $f(h_\theta(y))=y$ by construction, and hence problem \ref{} reduces to unconstrained optimization over $\Theta$:
% % \begin{equation}
% % h^*_\theta = \argmin_\theta \sum_Y \mathcal{L}(h_\theta(y))
% % \end{equation}
% Unfortunately, it is possible that there is no $\theta$ such that $h_\theta$ is optimal.
% % $h^*_\theta \neq h^*$.
% Suppose for example that $\mathcal{L}$ is such that the optimal inverse of $f(x) = x^4$ is $h^*(y) = -\sqrt[4]{y}$ when $y$ is even and $+\sqrt[4]{y}$ when $y$ is odd.
% We cannot derive $h^*$ using the parametric inverse $f^{-1}(y; \theta) = \theta \sqrt[4]{y}$ because for fixed $\theta$, its output is always positive or always negative.

% To remedy this, we must understand parametric inversion from an alternative perspective.
% A non-injective function is non-invertible because it lacks a unique inverse, but has multiple right-inverses. \todo{second second not implied by first.  f is a parametric representation of a space of right inverses because as you vary theta you get back different right inverse}
% Since for each fixed $\theta$ the function $f^{-1}(y; \theta)$ is a right inverse of $f$, $f^{-1}$ is therefore a parametric representation of a set of right-inverses of $f$, which we denote as $\mathcal{H}_{f^{-1}}$:
% \begin{equation}
% \mathcal{H}_{f^{-1}} = \left\{h_\theta \mid h_\theta(y)= f^{-1}(y; \theta \in \Theta) \right\}
% \end{equation}
% In the example, then $\mathcal{H}_{f^{-1}} = \left\{h_1(y) = \sqrt[4]{y}, h_2(y) = -\sqrt[4]{y}\right\}$, and the problem, plain to see, is that $h^* \notin \mathcal{H}_{f^{-1}}$.
% The solution is then to expand $\mathcal{H}_{f^{-1}}$.

% \begin{figure}[!htb]
% \label{fig:fib}
% \centering
% \includegraphics[width=0.95\linewidth]{funcspace.jpg}
% \caption{An Ali\=o program is a directed graph.}
% \end{figure}

% \subsection{Function Space Expansion}
% Composing a function approximator (such as neural network) between the inputs $Y$ and the parameters $\Theta$ expands the space of inverse functions a parametric inverse represents:
% % $$
% % \mathcal{H}_{f^{-1}} \subseteq \mathcal{H}_{f^{-1}_W}
% % $$
% \begin{algowizm}\label{n_y_w}
% Compose a function approximator $n: Y \times W \to \Theta$ with $f^{-1}$ to yield $f^{-1}_W: Y \times W \to X$ where $f^{-1}_W(y; \bm{w}) = f^{-1}(y; n(y; \bm{w}))$.
% \end{algowizm}

% $f_W^{-1}$ is a parametric inverse, but \emph{reparamterized} onto $W$ (the weight matrices of a neural network, for example), rather than $\Theta$. 
% Crucially, Reparameterization does not impact correctness:
% \begin{theorem}
% $f^{-1}$ is sound implies $f_W^{-1}$ is sound.

% \textit{Proof}.
% By definition in algorithm \ref{n_y_w}, $n(y; \bm{w}) \in \Theta$. Hence, $f^{-1}_W(y; \bm{w}) = f^{-1}(y; n(y; \bm{w}))$ is sound.
% \end{theorem}

% Reparameterization is not detrimental to completeness:

% \begin{theorem}\label{not-affect-completeness}
% Under mild conditions on $n$, if $f^{-1}$ is complete, $f^{-1}_W$ is complete.

% \textit{Proof.}
% See supplementary information.
% \end{theorem}

% % \begin{equation}\label{eq:g_property}
% % \end{equation}
% % MOVE TO SUPPL
% % \forall y \in Y, \forall \theta \in \Theta, \exists w \in W \text{, such that } g(y; \bm{w}) = \theta 
% % Condition \eqref{eq:g_property} is considered a mild assumption on $g$ because it is satisfied if $g$ is able to construct the constant functions for all the elements of $\Theta$.

% \rework{most importantly it expands the space of functions}
% It is essential to understand the importance of completeness of $f^{-1}$ in finding the optimal right inverse $h^*$. Suppose $f^{-1}$ is not complete so there exists $y$ and $x$ such that $f(x) = y$ but no $\theta$ satisfies $f^{-1}(y; \theta) = x$.
% This means that all the right inverses of $f$ that map $y$ to $x$ are excluded from $\mathcal{H}_{f^{-1}}$.
% With the incomplete parametric inverse $f^{-1}$, an optimal right inverse $h^*$ with $h^*(y) = x$ is not achievable, even with reparameterization.


% \begin{figure}
%   \centering
%     \includegraphics[width=0.4\columnwidth]{sub_arrow_heatmap.pdf}
%     \includegraphics[width=0.4\columnwidth]{inv_fwd_heatmap.pdf}
%   \caption{A comparison of $\mathcal{L}^2$ (top) and $\mathcal{L}^1$ (bottom) on the parametric inverse of $f(x,y) = xy+x$. The two surfaces impose different optimization characteristics.}\label{fig:diffloss}
% \end{figure}

% \section{Parameter Generating Functions}\label{pgf}
% \rework{Motivate why we need parameter generating function}
% From $x$, a parameter generating function constructs a parameter $\theta$ such that $f^{-1}(y; \theta) = x$, where $y=f(x)$.

% \begin{definition}$r: X \to \Theta$ is a parameter generating function of a parametric inverse $f^{-1}$ if for all $x$:
% \begin{equation}
% f^{-1}(f(x); r(x)) = x
% \end{equation}
% \end{definition}

% For example, $f^{-1}(y; \theta \in \{-1, 1\}) = y \cdot \theta$ is a parametric inverse of absolute value, and $r(x) = \operatorname{sgn}(x)$ is a valid parameter generating function, where $\operatorname{sgn}(x):=1$ if $x>0$ and $-1$ otherwise.

% A function is a parameter generating function only with respect to a particular parametric inverse, and even then, may not be unique.
% Continuing the previous example, it is equally valid for $r(0)=1$ rather than $r(0)=-1$.
% More generally, a parameter generating function is unique only if there is a unique correspondence between parameter values and elements of the preimage.

% % \begin{definition}A parametric inverse $f^{-1}$ is bijective if for all $y \in Y$,
% % $f^{-1}(y; \theta)$ is a bijection between $\Theta$ and $X$.
% % \end{definition}

% Parameter generating functions of composite parametric inverses can be derived compositionally.
% Let $f=f_1 \circ f_2$ and $f^{-1} = f_2^{-1} \circ f_1^{-1}$, be its parametric inverse whereby $f^{-1}$ is the parametric inverse of $f_1$.
% Let $r(x) = (r_1(x), r_2(x))$, then $r(x)$ is a parameter generation function for $f^{-1}$.

% % Parametric inverse may not have this simple form.
% % For example if the one parameter value is a function of another.
% % Deriving parameter generating function of these compositions is more complex.
% % However it won't make much difference in the end.
% % \todo{Section on Implementation: what would I need to know in order to get it to work.  autodiff, optimization, }

\section{Ali\=o: An Inverse Simulation Framework}\label{alio}
Our treatment of inversion has so far been purely in terms of mathematical functions; we extend it now to Ali\=o dataflow graphs.
Ali\=o consists of tools to (i) construct an Ali\=o graph or derive it from imperative (Julia) code, (ii) construct its parametric inverse, also as an Ali\=o graph, and (iii) compile it back to either imperative Julia code or TensorFlow graphs for optimization.

Dataflow graphs model computation as a directed graph of data flowing between operations.
They were most actively explored in the 1970s and 1980s \cite{Johnston2004}, but have recently regained prominence within machine learning and inference frameworks such as Theano and TensorFlow \cite{Bergstra2010, Agarwal2015}.

\subsection{Specification}
An Ali\=o dataflow graph is a directed, bipartite, multigraph $G=(V,E)$, composed of \textit{op} and \textit{value} nodes.
Let $\vmn$ denote a node which receives $m$ edges and projects $n$ edges, ordered from 1 to $m+n$.
We refer to a pair $(v, i)$ as a \textit{port}, and therefore $E$ is a relation over ports.

Each value node receives exactly 0 or 1 edge.
If a value node receives 0 edges it must be labeled as an input or constant.
If a value node projects 0 edges it must be labeled as an output.
An op node models a multi-input, multi-output function, and hence receives at least 1 edge and projects at least 1 edge.

% \subsection{Denotational Semantics}
% A well formed dataflow graph denotes a function.
% \rework{DO denotational semantics

\subsection{Constraint Solving}

Let $f: Y \times \Theta \to X$ be a partial parametric inverse of $f: X \to Y$, and $\Theta = \Omega_1 \times \cdots \times \Omega_n$ be a product space of $n$ components.
Let $C = c_1, \dots c_n$ be a set of constraints derived from symbolic execution.
Each constraint has the form
$$
c_i: V_i \to \{0, 1\}
$$
Where $V_i$ is a set of variables (to be defined shortly).
For a given set, e.g., $\Theta_1 \times \cdots \times \Theta_n$, let $\pi_{i,...,k}(\Theta), $ denote the projection of $\Theta$ to $\Theta_i \times \cdots \times \Theta_k$: its $i,..,k$th components.
$V_i$ is then the set of variables.

By the partiality theorem of parametric inversion: for any $y$ in the image of $f$, let $x = f^{-1}(y; \theta)$, $x$ is a valid inverse of $y$ (i.e., $f(x) = y$) if and only if, for all $c_i$:
$$
\bigwedge\limits_{i=1,...n} c_i(y, \theta)
$$
That is, all the constraints are satisfied.

To solve constraints means to construct (i) a new parameter space $\Theta hat$, and (ii) a function $g:Y \times \Theta \to \Theta$ such that the constraints are satisfied.
More precisely, let $A \subset Y \times \Theta$ be the totalizing subset, i.e. the preimage $f^{-1}(A) = X$, and in particular $\bot \notin f^{-1}(A)$, construct $g$ such that $g(Y\times \theta_{hat} = A$.

Finally, we assume $\Theta_{hat}$ is nice, in the sense that it is easy to span (can we formalize this?)

Let's focus on the case where $\Theta_{hat}$ is made of, i.e. a projection of $\Theta$.
Suppose we partition $\Theta$ into two products $\Theta_{ind}$ and $\Theta_{dep}$ denoting independent and dependent variables.

\subsection{Compilation}
Ali\=o currently compiles both to imperative Julia and TensorFlow.
TensorFlow is also a dataflow framework and hence compilation from Ali\=o is straightforward, save the following caveats.
TensorFlow has no support for composite functions and hence an Ali\=o program must first be flattened, such that every node within a composition is primitive.

Compilation to imperative code is more involved.
We assume any primitive arrow will be implemented in the host language.
\todo{finish the sentence here}
This is made considerably more complex if there is conditional flow in the graph because we must ensure that given what is known about the condition branch of an \inlinecode{IfThenElse} node, we only compute necessary values.
Section \ref{sec:compilation} of the supplementary provides a precise algorithm.

\subsection{Limitations}
Ali\=o does not support higher order functions.
Fortunately, much of the utility of higher order functions can be taken advantage from within Julia in construction of the Ali\=o graph.

Ali\=o supports conditional branching but currently has parametric inversion defined only for functional non branching \inlinecode{IfThenElse} nodes.
Parametric inversion of branching conditional flow is also feasible as a graph transformation, but cannot be done on a node by node basis as our algorithm currently operates.

Finally Ali\=o programs are purely functional.
It is not meaningful to invert programs which cause side effects, and hence these are omitted by design.

\subsection{Propagation of Types, Shapes and Values}
\label{propagation}
Ali\=o has a unified framework for propagation of different kinds of values around the dataflow graph.
Constant propagation is a compiler method to statically infer constant values, and has even greater utility in parametric inversion, because if one or more inputs to a multi-argument function are constant, its inverse will have fewer or even zero parameters.
For example, the parametric inverse of addition $+^{-1}$ takes a single parameter, but is invertible if either input is constant.
The savings in complexity are substantial for programs which manipulate arrays: when the indices used to index an array are known to be constant, as is often the case, its parametric inverse has significantly fewer parameters.

Shape inference \cite{joisha2006algebraic} means to infer the dimensionality of multidimensional arrays, often used to optimize memory allocation and prevent errors.
Frameworks such as TensorFlow and Theano have specialized shape propagation algorithms.
Shape propagation is particularly important in parametric inversion of array based Ali\=o programs, because the shapes of the parameter inputs are not under the user's control and infeasible to derive manually.

% Ali\=o has a single framework for propagation of all of these types of information based on abstract interpretation \cite{Cousot1977, Cousot2001}.
% We view the type, shape and constancy as abstractions of a particular value.
% The following is a sketch of the propagation algorithm; in section X we provide a more precise procedure.
% \todo{where is the sketch and what section?}

\subsection{Extra Details}
Ali\=o is an extensive framework.  Here we touch briefly upon implementation details:

\emph{Host Integration:}
There are three methods to construct an Ali\=o program within Julia.
The first is to use the primitive graph transformations to construct empty graphs, add nodes to graphs, link nodes within a graph, and compose graphs together.
This can be cumbersome, so the second method relies on overloading primitive operators such as $+$ and $-$ to be defined on Ports as if they were values.
A problem with this approach is that you lose information about the composition of the graph.

\emph{Optimization:}
Optimization is done in TensorFlow, and NLopt.
Gradients are derived with automatic differentiation.

\section{Parametric Inversion of Ali\=o Programs}\label{invertalio}
Parametric inversion of Ali\=o graphs brings a number of complexities over simple functions.

\subsection{Duplication of Values}\label{dupl}
One problem that arises in programs is the reuse of values.
The reuse of values presents no problem in the forward computation but can be problematic in the inverse.
For example it is easy to compute $f(x,y) = xy + x$, but depending on the parameter values, $+^{-1}$ and $\times^{-1}$ may produce two different, and hence conflicting values for $x$.

In a dataflow graph, $n > 1$ implies a vertex $\vmn$ is reused.
Before inversion, we eliminate reuse of values with use of a function $\dupl$, which duplicates its input $\dupl_n(x) = (x,..,x)$.
For each $\vmn$ where $n>1$, we add a $\dupl_n$ op node and $n$ value nodes to $G$.
Then, we replace all outgoing edges from $\vmn$ with a single edge to $\dupl_n$ and project from $\dupl$ to each new vertex, and from each vertex to its original destination.

$\dupl$ is invertible, and hence its inverse does not require parameters.
The domain of its inverse expects two identical inputs, and $\dupl^{-1}(x,y) = \bot$ if $x \neq y$.
With $\dupl$, reuse of values is no different from the domain constraints outlined in the previous sections.
It causes partiality, and can be treated with the same methods.
An unsound but total $\dupl^{-1}(x,y) = x$ simply outputs $x$ and ignores $y$.
In all our examples $x,y \in \mathbb{R}^n$; we instead take the mean: $\dupl^{-1}(x, y) = \mean(x, y)$.
Both are permissible under the conditions of algorithm 2.

\subsection{Array Primitives}
Ali\=o provides a number of primitive functions for working with arrays, and their corresponding parametric inverses.
For indexing, we follow the TensorFlow/numpy model with $\gathernd(x, \iota)$ and $\scatter(z, \iota, \sigma)$. $\gathernd(x, \iota)$ constructs a new array taking the elements from $x$ in the order provided in $\iota$. $\scatter(z, \iota, \sigma)$ creates a new array shaped $\sigma$ initialized with zeros, and stores at indices $\iota$ the values taken from $z$. If $\iota$ and $\sigma$ are constants, $\scatter^{-1}(z, \iota, \sigma) = \gathernd(x, \iota)$, but $\scatter(z, \iota, \sigma)$ is not the inverse of $\gathernd(x, \iota)$. Notice that in order to compute $\gathernd^{-1}(x, \iota)$, it requires parameters $\theta$ and $\sigma$, but in practice the latter can be inferred using shape propagation. Then $\gathernd^{-1}(x, \iota, \sigma, \theta) = \scatter(z, \iota, \sigma) + \theta$.

Ali\=o also provides $\reshape(x, \sigma)$, where $x$ is the input array and $\sigma$ is the output's shape. In the case where the shape can be inferred using shape propagation, $\reshape$ is invertible: $\reshape^{-1}(x, \sigma) = \reshape(z, \tilde{\sigma})$.

% \todo{is this necessary? or can anyone finish it?}
% Finally, Ali\=o provides support for array reduction along an axis, which allows the dot product.  Its parametric inverse

\subsection{Dataflow Program Inversion}

To transform $G$ into its parametric inverse $G^{-1}$ we generalize algorithm \ref{algo:compinversion} to graphs.
To construct $G^{-1}$, we (i) relabel each input node as an output node and vice-versa, (ii) substitute each primitive op node with its corresponding parametric inverse op node, and (iii) invert the direction of the edges.
% Algorithm X in the supplementary material provides a precise algorithm for this transformation.
Algorithm \ref{alg:pi-dataflow-local} constructs an inverse dataflow graph $G^{-1}$ from the forward graph $G$.
It relies on a function $\invmap$ which maps port on an op to ports on its inverse.

\setcounter{algorithm}{2}
\begin{algorithm}[H]
   \caption{Parametric Inversion of Dataflow Graph}
   \label{alg:pi-dataflow-local}
\begin{algorithmic}
   \STATE {\bfseries Input:} graph $G$
   \STATE {\bfseries Output:} graph $G^{-1}$
   \STATE Initialize $G^{-1} = (V^{-1}, E^{-1})$ as empty graph
   \STATE Initialize $m$ to empty mapping from ports in $G^{1}$ to $G^{-1}$

   
   \FOR{$v$ {\bfseries in} value nodes of $V$}
   \STATE Add $v^{-1}$ to $V^{-1}$
   \IF{$v$ is output} 
   \STATE Label $v^{-1}$ as input
   \ELSIF{$v$ is input}
   \STATE Label $v^{-1}$ as output
   \ENDIF
     \FOR{$i=1$ {\bfseries to} $n$}
       \STATE Assign $(v, i)$ to $(v^{-1}, i)$ in $m$
     \ENDFOR
   \ENDFOR
   
   \FOR{$o$ {\bfseries in} op nodes of $V$}
   \STATE Add $o^{-1}$ to $V^{-1}$
   \STATE Update $m$ with all values from $\invmap(o, o^{-1})$
   \ENDFOR
   
   \FOR{$l, r$ {\bfseries in} $E$}
   \STATE $l^{-1} \gets m(l)$
   \STATE $r^{-1} \gets m(r)$
   \IF{$l^{-1}$ is output} 
   \STATE Swap $l^{-1}$ and $r^{-1}$
   \ENDIF
   \STATE Assign $l^{-1}$ to $r^{-1}$ in $E^{-1}$
   \ENDFOR
   \STATE \textbf{return} $G^{-1}$; all unconnected ports are parametric inputs
\end{algorithmic}
\end{algorithm}

\begin{theorem}
\label{thm:soundcompletegraph}
$G^{-1}$ is a sound and complete parametric inverse of $G$.

\textit{Proof.}
See supplementary information.

\end{theorem}


\subsection{Parameter Reduction}\label{paramreduction}
In section \ref{unsoundtotal} we described a method to totalize any partial parametric inverse, but the result may be unsound.
Here we present a method to reduce the number of parameters which does not compromise soundness.

First we derive a symbolic expression for $A \subset \Theta$: the constrained set on which $f^{-1}(y;\theta \in A) \neq \bot$.
In particular, we derive $A$ as a \textit{refinement type} \cite{All the people} of the form $\{\nu:B \mid e\}$, where $\nu$ is a special value variable, $B$ is a base type and $e$ is a refinement predicate: a boolean-valued expression which constraints the value variable.
For example:
$$
\theta: \left\{\nu : \mathbb{R} \mid \nu \ge 0 \right\}
$$
With refinement types, the derivation of $A$ is a form of type inference, which we achieve using a symbolic execution of the program:

\setcounter{algorithm}{3}
\begin{algorithm}[H]
   \caption{Parameter Reduction}
   \label{algo:refinement}
\begin{algorithmic}
   \STATE {\bfseries Input:} an Ali\=o program $P$.
   \STATE {\bfseries Output:} A set of constraints on parameters.
   \STATE For each function $f$ create symbolic counterpart $\tilde{f}$
   \STATE Create symbolic arguments $x_1^1, x_2^1, \dots, x_n^1$. 
   \STATE Add shape information to arguments from shape propagator's algorithm.
   \FOR{$\tilde{f}^i$  {\bfseries in}  $P$, in evaluation order}
   \STATE 	Symbolically interpret $\tilde{f}^i(x_1^i, x_2^i, \dots, x_{n_i}^i) = \alpha^i$.
   \STATE Compute domain predicates $\delta^i$ for $\tilde{f}^i$ given  $x_1^i, x_2^i, \dots, x_{n_i}^i$.
   \STATE Define new refined symbol $\tilde{\alpha}^i := \{\alpha^i | \bigcup_{j=1}^{n_i} \text{pred}(\tilde{x}_j^i)\}$.
   \ENDFOR
   \STATE For constraints of the form $\theta_i = \gamma(\theta_j, \theta_k, \dots)$,
   \STATE add new functions $\hat{h}: \theta_j \times \theta_k \times \dots \to \theta_i$.
\end{algorithmic}
\end{algorithm}


\subsection{Parameter Elimination}\label{elimination}
Depending on $f^{-1}$, solving the constraints derived from the symbolic execution may be hard or even undecidable.
In this work, we focus purely on eliminating parameters.
That is, given the constraints of the form $\theta_i = \gamma(\theta_j, \theta_k, \dots)$, for a function $f$ and arguments different to $\theta_i$, we (i) infer the minimal number of parameters, and (ii) rewrite the Ali\=o program onto this reduced space.
We create a new function $h$ from the reduced space onto the space of $f^{-1}(y, \theta \in A)$, and so it can be composed with $f^{-1}$. This function $h$, will rewire the parameters and apply transformations to them to satisfy the constraints. 

For arrayed variables, constraints may involve indexes, for which it's necessary to first use $\gathernd$ to pick  the relevant elements from each parameter, apply the required transformation $\gamma$, and reconstitute the array with a combination of $\scatter$ and element-wise additions. 
Furthermore, in some cases,  constraints of the form $\psi(\theta_i) = \gamma(\theta_j, \theta_k, \dots)$ can also be solved. In particular, when $\psi^{-1}(\cdot)$ is a total function, Ali\=o can be used to compute $\psi^{-1}(\cdot)$ and apply it to $\gamma$ before the use of $\scatter$.

\subsection{Summary of Procedures}
Given a Ali\=o program $f: X \to Y$, we:
\begin{itemize}
\item Infer type, shape, and constancy information of $f$ (Section \ref{propagation})
\item Derive a partial parametric inverse $f^{-1}:Y \times \Theta \to X$ (algorithm \ref{alg:pi-dataflow-local})
\item Derive constraints on $\Theta$ as a refinement type (algorithm \ref{algo:refinement})
\item Eliminate redundant parameters (Section \ref{elimination}) to yield a new parameter space $\Theta'$.
\item If $\Theta'$ remains constrained (inferred by repeating step 2), perform an unsound totalization using the contractors (algorithm \ref{algo:contraction})
\item From $\apinv{f}$ construct the domain loss $\mathcal{L}_{dm}$ which measures the degree to which the constraints of $\Theta$ are violated for some input (Section \ref{unsoundtotal})
\end{itemize}

$\apinv{f}$ can be used to solve the inverse problem \eqref{eq:inverseproblem} described in the introduction.
Rather than search over $X$, we search over $\Theta$.  For a target value $y$ we wish to invert, we find $\theta^*$:
\begin{equation}\label{eq:optinverseproblem}
\theta^* = \argmin_\theta \mathcal{L}(\apinv{f}(y; \theta), y) + \mathcal{L}_{dm}(\apinv{f}; y, \theta)
\end{equation}
then:
\begin{equation}
x^* = \apinv{f}(\theta^*)
\end{equation}
% $\apinv{f}$ can be used to address the inverse problem mapping problem \eqref{eq:inverseproblem}, \eqref{}.
% \begin{itemize}
% \item Compose $f^{-1}$ with a neural network.
% \end{itemize}

% \begin{equation}
% \bm{w}^* = \argmin_{\bm{w}} \sum_{y \in Y} \mathcal{L}(\apinv{f}(y; \bm{w}), y) + \mathcal{L}_{dm}(\apinv{f}; y, \bm{w})
% \end{equation}
% then for all $y$:
% \begin{equation}\label{eq:optinversemap}
% h^*(y) = \apinv{f}(y; \bm{w})
% \end{equation}
\section{Micro-evaluation}\label{microanalysis}
In this section we investigate properties of parametric inverse with a number of small benchmarks.

\subsubsection*{Initialization Hypothesis}
As we have discussed, the parametric inverses we construct are typically partial.
There are two ways in which using a parametric inverse can change optimization characteristics.  First, the structure of the function $f^{-1}$ may bias us towards (or away from) solutions  The loss surface over $\Theta$ compared with over $X$ may be more or less tractable. 
To test this we examine the distribution over (identity) loss values both prior to and after optimization and compare optimization over $\Theta$ and $X$.
In figure \ref{init} we show results from two representative functions and in table \ref{compareopt} we show aggregate results over all random examples (Section \ref{random} of supplementary information). 

\begin{figure}[!htb]
\centering
\includegraphics[width=0.95\linewidth]{histinit2}
% \includegraphics[width=0.45\linewidth]{losshist.png}
\caption{Comparison of losses at initialization}\label{init}
\end{figure}

\begin{table}[h]
\resizebox{\linewidth}{!}{%
\begin{tabular}{r|ccccc}
	& Test & pre-mean & pre-var  & init-mean & init-var\\
	\hline
	1 & $\Theta$ & 0.0120237 & 0.000998488 & 6.85907e5 & 6.54375e28 \\
	2 & $X$ & 0.253715 & 0.167953 & 3.01392 & 560.138 \\
\end{tabular}
}
\medskip
\caption{Aggregate results over all random examples}\label{compareopt}
\end{table}

Both figure \ref{init} and table \ref{compareopt} show that both approaches initialize with similar distributions over loss, although the parametric inverse has a very higher variance.
This 
However a parametric inv


\subsubsection{Comparison of Loss Functions}
There are two possible loss functions to use with a parametric inverse, discussed in section \ref{unsoundtotal}.
The domain loss is more fined grained, in the sense that it is the accumulation of loss functions of each primitive.
One of the problems of naive optimization is sparsity of the solution set.
One hypothesis then is that by decomposing the loss term into many small ones which can be solved more readily, the domain loss induces an optimization surface more amenable.
Of course it is more expensive to compute, since error terms are computed after every primitive operation.

\begin{figure}[!htb]
\centering
%\fbox{\includegraphics[width=0.45\linewidth, trim={.2cm, .3cm, .15cm, .20cm}, clip]{losshist.png}}
\includegraphics[width=0.45\linewidth, trim={.2cm, .3cm, .15cm, .20cm}, clip]{losshist.png}
%\fbox{\includegraphics[width=0.45\linewidth, trim={.2cm, .3cm, .15cm, .20cm},, clip]{losshist.png}}
\includegraphics[width=0.45\linewidth, trim={.2cm, .3cm, .15cm, .20cm}, clip]{losshist.png}
\caption{Comparison of $\mathcal{L}_{id}$ and $\mathcal{L}_{dm}$}
\end{figure}

\begin{figure}[!htb]
\centering
\includegraphics[width=0.95\linewidth, trim={.2cm, .3cm, .15cm, .20cm}, clip]{domloss}
\caption{Comparison of $\mathcal{L}_{id}$ and $\mathcal{L}_{dm}$}
\end{figure}

\section{Evaluation}\label{evaluation}

% \subsubsection{Hypothesis}
% Using parameters of PGF places us closer to conditional distribution of parameters
% Given a distribution over $X$The optimal initialization distribution over parameters if 
% If the distribution over $X$ is unknown, it is still preferable to initialize $\theta$ with an arbitrary distribution over $X$ and generate parameter values with a pgd than to choose an arbitirary distribution over $\Theta$ directly

% \subsubsection{Structural Prior Hypothesis}
% A parametric inverse imposes a structural prior on a space of functions which is closer to the posterior than an unconstrained neural network.


% \subsubsection{Function Space Warping Hypothesis}
% Any parameterized function expresses a space of functions.
% Increasing the number of weights in a neural network is thought to both increase its information capacity and its expressivity: the complexity of the functions it contains.

% Our goal is to understand how the function space expressed by a neural network changes when it is composed with a parametric inverse.
% The hypothesis is that composing a neural network with a parametric inverse warps

% f a a neural network A parametric inverse warps the space of functions that are parametrically represented by a neural network.
% Similarly a neural network expands the set of right inverses induced by a neural network.

We evaluated parametric inversion on two real problems:

\textbf{Inverse Rendering}: We invert a function which renders voxels into an image.
The renderer simulates a diffusely illuminated emission-absorption optical model \cite{Hadwiger2009}, which uses two scalar-fields to represent geometry.
$\kappa(\mathbf{x}) \in \mathbb{R} \text{ with } \mathbf{x} \in \mathbb{R}^3$ represents the attenuation coefficient at each point in space (accounting for the absorption of light), while $c(\mathbf{x})$ are the emissive colors (accounting for actively emitted radiant energy).
For each pixel, the forward rendering function casts a single ray from the eye through the volume, and integrates optical properties along the way to find the incident energy $C$:
$$
C = \int_0^\infty c(t) \cdot e^{-\int_{0}^{t} \kappa(t)}\\
$$
Where $c(t):=c(\mathbf{x}(t))$ and $\kappa(t):=\kappa(\mathbf{x}(t))$ denote optical properties at distance $t$ along a parametric ray $\mathbf{x}(t)$.
A parametric inverse constructs $c$ and $\kappa$ from an image.

\begin{figure*}
\includegraphics[width=\linewidth]{inv_renderer.png}
\caption{Consistency results for inverse rendering. The left image of each triple shows our forward renderer's output given a voxel grid. For the first 6 examples, we infer parameter values from this forward run, which we use to invert the output. These parameters are computed by simply propagating corresponding parameter values from each primitive during the forward execution. The middle image results from viewing the inverted output with the same forward renderer. The right image results from viewing the inverted output at a different angle. In the last two examples, we arbitrarily set all parameters to 1 to show that the reconstruction works only for the front view without correct parameters.}\label{inv_renderer}
\end{figure*}


\textbf{Inverse Kinematics}: Inverse kinematics computes joint configurations of a robot consistent with its end-effectors reaching a desired position.
To compute inverse kinematics we parametrically invert the forward kinematic function of a 6 degree-of-freedom Stanford robot arm whose forward kinematics are specified in \cite{Kucuk2006} in Denavit-Hartenberg convention.

\textbf{Random Problems}: To evaluate more exhaustively, we randomly generated problems by defining a sampling process (see supplementary information) over primitives in table \ref{tab:inverses}.

\subsection{Experimental Setup}

Ali\=o is intended to be a drop in replacement for optimization in complex inverse problems and hence our evaluation is straightforward.
As stated in the introduction, we compare optimization over $X$ using the forward function with optimization over $\Theta$.

% \textit{1. A right-inverse $h_W$ induced from a parametric inverse $f^{-1}$ reparameterized with a neural network $g_1: Y \times W \to \Theta$.}
% To construct $h_W$ we: (i) implemented $f$ as a TensorFlow graph, (ii) constructed a parametric inverse $f^{-1}$ using algorithm 3, (iii) assuming $f^{-1}$ is partial, used algorithm \ref{algo:contraction} to construct its totalized counterpart $\apinv{f}$, and (iv) used a neural network $g_1$ to expand $\apinv{f}$ to yield $\apinv{f}_W$ and induce a right-inverse $h_{{\bm{w}}}(y) = \apinv{f}_W(y; \bm{w}) = \apinv{f}(y; g_1(y; \bm{w}))$. 
% %\todo{This equation is wrong, g is missing}

% \textit{2. A neural network $g_2: Y \times W \to X$.}

% The concrete loss function we minimize is the least squares error over a dataset of $(y, x)$ examples, i.e., in both cases we seek an optimal $h^*_{\bm{w}}$:
% \begin{equation}
% \argmin_{\bm{w}} \sum_i \norm{\hat{x}_i - x_i}^2 + \norm{f(\hat{x}_i) - y_i}^2 \ \text{ where } \ \hat{x}_i = h_{\bm{w}}(y)
% \end{equation}

% \textbf{Tests:} We compared test and training error, varying the dataset in the inverse kinematics example (table 2), and fixed the dataset for the random graphs to compare training dynamics (Figure 3: Right).
% We parametrically inverted a 3D renderer but did not find an optimal inverse mapping.

% \textbf{Data:} In all  examples, from a dataset $x_i,\dots,x_n$, we generated $n$ pairs $(f(x_i), x_i),\dots,(f(x_n), x_n)$ using the forward model.
% In both inverse kinematics and the random functions, $x_i$ were sampled uniformly from $X$.
% For rendering, we converted ModelNet40 \cite{Wu2015} dataset into voxel grids of dimension $32 \times 32 \times 32$, and using $f$ generated $128 \times 128$ pixel images from a fixed orientation.

% \textbf{Network Structure: }
% We used residual networks \cite{He2016} of block size 2 with ELU  \cite{Clevert2015} activation units.
% In inverse kinematics and the rendering example, fully connected layers were used for each layer within the residual block.

% \textbf{Network Matching: }
% For fair comparison, in all examples we match the structure of $g_2$ to $g_1$.
% Precisely matching $g_2$ to $g_1$ has no perfect solution because the codomains may have different dimensionality ($X$ and $\Theta$ respectively).
% Our solution was to adjust the number of residual blocks to match as closely as possible the number of parameters within the two neural networks.

% \textbf{Optimization Hyper-Parameters: }
% The forward renderer was implemented in TensorFlow.
% We trained with the ADAM optimizer \cite{Kingma2014} (with $\beta=0.5$), with a learning rate of 0.01, and a minibatch size of 32.
% Weights were initialized with the method from \cite{Glorot2010}.

% \noindent\begin{minipage}{\linewidth}
% \centering
% \includegraphics[width=0.4\linewidth]{allthreegood.png}
% \captionof{figure}{Example figure caption (non-floating)}
% \label{fig:examplenf}
% \begin{table}\label{table:res}
%   \centering
% % \resizebox{\textwidth}{!}{%
%   \begin{tabular}{ c | c | c | c | c }
%   	$D$ & PI Train Error & NN Train Error & PI Test Error & NN Test Error \\
%     \hline
% $1$ & $\textbf{0.28; 0.09}$ & $0.33; 0.2$ & $\textbf{0.35; 0.1}$ & $0.51;0.143$ \\
% $7$ & $0.13; 0.01$ & $\textbf{0.1; 0.014}$ & $\textbf{0.19;0.014}$ & $0.235;0.01$ \\
% $15$ & $\textbf{0.08;0.004}$ & $0.1;0.0125$ & $\textbf{0.14;0.005}$ & $0.24;0.014$ \\
% $25$ & $\textbf{0.11;0.009}$ & $0.13;0.014$ & $\textbf{0.2; 0.019}$ & $0.25;0.022$ \\
% $36$ & $0.21;0.013$ & $\textbf{0.16;0.033}$ & $0.25;0.014$ & $\textbf{0.234;0.04}$ \\
% $50$ & $\textbf{0.12;0.009}$ & $0.18;0.027$ & $\textbf{0.19;0.014}$ & $0.33;0.046$ \\
% $70$ & $0.1; 0.005$ & $\textbf{0.07;0.002}$ & $\textbf{0.2; 0.015}$ & $0.29;0.039$ \\
% $90$ & $\textbf{0.2; 0.017}$ & $0.35; 0.17$ & $\textbf{0.25; 0.02}$ & $0.46; 0.14$ \\
% $120$ & $0.286;0.15$ & $\textbf{0.27; 0.18}$ & $\textbf{0.38;0.154}$ & $0.42; 0.13$ \\
% $150$ & $\textbf{0.12; 0.01}$ & $0.24; 0.15$ & $\textbf{0.22;0.014}$ & $0.38; 0.16$ \\
%     \hline
%   \end{tabular}
  
% %   }
% 	  \caption{Table of results from inverse kinematics. mean;variance of train/test error of a model trained on a dataset of size $D$ for $N=5000$ iterations. Each experiment was run 10 times.}\label{tab:results}
% \end{table}

% \begin{table}\label{table:testtrain}
% \begin{tabular}{r|cccc}
% 	& D & pi\_pgf\_dom & pi\_pgf\_id & net\\
% 	\hline
% 	1 & 1 & 0.152566 & 0.023184 & 0.847994 \\
% 	2 & 2 & 0.382403 & 0.298525 & 0.211862 \\
% 	3 & 3 & 0.129746 & 0.99321 & 0.551495 \\
% 	4 & 4 & 0.420278 & 0.757962 & 0.906369 \\
% 	5 & 5 & 0.137574 & 0.121731 & 0.0659937 \\
% 	6 & 6 & 0.184616 & 0.378846 & 0.509289 \\
% 	7 & 7 & 0.339822 & 0.810603 & 0.272078 \\
% 	8 & 8 & 0.8285 & 0.776381 & 0.11823 \\
% 	9 & 9 & 0.948776 & 0.986657 & 0.876689 \\
% 	10 & 10 & 0.187754 & 0.36986 & 0.362292 \\
% \end{tabular}
% \end{table}


\subsection{Analysis}
Parametric inversion consistently outperformed an unconstrained neural network in terms of generalization (table 2).
One hypothesis is that the parametric inverse imposes a stronger structural prior over inverse functions.
In terms of training error the parametric inverse trained faster, and slightly outperformed the unconstrained network.
Both $g_1$ and $g_2$ must solve the optimality problem, but in addition, $g_2$ must reconstruct the inverse mapping, essentially given by the parametric inverse for free.
Of course, $g_1$ must solve the partiality constraints, which in a minority of cases is a more difficult task than the inverse problem itself.

Although we successfully parametrically inverted the ray-tracing renderer figure \ref{inv_renderer}, numerical instabilities prevented optimization of $h^*$.
This is due to a cascade of inverse multiplications and exponentiations in $f^{-1}$, which easily cause an explosion in gradients.
This highlights the fact that for functions such as these, totalization is insufficient.
In addition, we need to ensure we initialize and remain in a stable part of the parameter space; this is a task for future work.

% \begin{figure}
% \centering
% \includegraphics[width=0.4\linewidth]{error_vs_datasize.pdf}
% \includegraphics[width=0.4\linewidth]{allthreeno2.pdf}
% \caption{(Left) Size of training dataset vs test and training error in inverse kinematics.
% (Right) Test error vs time during training. Each approach trained on 50 randomly sampled graphs.  Upper, middle, and lower boundaries denote upper quartile, median and lower quartile of error.
% }\label{error-vs-datasize}
% \end{figure}

% Parametric inverse methods learned inverse mappings typically faster, to lower test error (\ref{time-error-compare}) and with better generalization (figure \ref{error-vs-datasize}) than function approximation.


% Technically, our approach bears most resemblance to interval constraint propagation (ICP) \cite{Granvilliers2006a}\todo{fix citations, here and in rest of section}, which solves problems of the form $f(x)=0$.
% A parametric inverse varies over points in the preimage of value.
% In contrast, ICP \emph{contracts sets}, represented as intervals, to be closer to the preimage of a value.
% Using sets instead of points allows ICP methods to be sound and complete in the sense that if an $x$ exists it will be found.
% The effectiveness of ICP is limited by the extent to which it can find good contractions, which is particularly poor for functions with multiple reuse of the same variable.

% Another approach is to encode the forward function into a language that is fully reversible by construction.
% Reversible languages such as \cite{Mu2004,Alimarine2005} simply disallow non-injective functions.
% Perhaps surprisingly, \cite{Bennett1973} and further explored in \cite{Axelsen2011a} show that reversible models of computation can encode any computation that non-reversible ones can.
% In some sense, a parametric inversion encodes a non-invertible function into an invertible form (through the parameter); hence our approaches are similar.

% \subsection{Future Work}


Parametric inversion involves both symbolic reasoning and learning for reparameterization. Our current relatively simple symbolic reasoning could benefit from additional program analysis techniques to optimize $f^{-1}$ prior to reparameterization.  One way to view the dynamic is that each improvement on the symbolic side makes the learning task for $g$ easier by reducing the partiality constraints.


\section{Related Work}
Program inversion has a long albeit scattered history.
McCarthy \cite{McCarthy1956} proposed to invert Turing machines which test whether a candidate solution to a given problem is correct.
Dijkstra \cite{Dijkstra1979a} and Gries \cite{gries2012science} manually derived inverses of imperative programs by step by step inversion of each operation.
Subsequent approaches automate this step-by step principle: \cite{Gluck2003, Gluck2004}.  \cite{hu2017automatic} invert each transition of a restricted class of symbolic extended finite transducers; we (parametrically) invert each primitive within compositions.
These approaches, with the exception of parametric inversion, apply to injective functions defined on discrete domains.
Proving that a program is invertible is itself nontrivial (and generally undecidable \cite{hu2017automatic, Fulop1994}). \cite{Gluck2003} for example requires the program to be structured such that the compiler can prove that it is injective.

Non-invertibility has been addressed in a number of ways.
Approaches based on logic programming such as \cite{Ross1997} view of an imperative program as a relation.
\cite{Abramov2002, harrison1992synthesis, khoshnevisan1989invx, Nishida2011} define inversion semantics in terms of the power domain; an inverse function then returns the set of all inputs which map to a particular output.
Such methods, sometimes referred to as full or universal, are in contrast with partial or existential methods which return a single result.


While most methods (including parametric inversion) deductively derive an inverse program, \cite{srivastava2011path} treats program inversion as a form of inductive program synthesis, employing SMT (satisfiability modulo theories) solvers to synthesize an inverse program.
Despite recent advances \cite{Gao2012}, SMT solving over non-linear functions is limited, and hence their method has not been applied to the kinds of problems found in machine learning, vision, robotics, etc.

% Program inversion sometimes refers to the undoing of computation in editors, transaction systems, and reverse debugger \cite{Feldman1989}s.
% In contrast, the problems which motivate this contribution do not have the benefit of a partially executed program forward program.

Program inversion appears in a much wider range of fields, often in disguise.
Deep neural networks have seen some success in inverting conventional programs, typically from input-output example pairs generated from simulation.
The increasing sophistication of deep neural networks has blurred the distinction between conventional programs and function approximators.
% Function inversion is a fundamental principle in mathematics and model inversion is a central part of.
% Inverse problems have extensive history in the natural sciences.
% The dominant approach is to use gradient based optimization to search for the inverse of an observed value \cite{tarantola2005inverse}.
% The advantage of this approach is that the function can be black-box; we need only the ability to evaluate it (and possibly its derivative) on particular inputs.

Program inversion has deep connections to probabilistic inference.
If a mathematical model is represented as a function from causes to observations, its non-injectivity precisely manifests any and all uncertainty in the model.
The regularization technique introduced in the introduction (and used heavily in so called inverse problems \cite{tarantola2005inverse}) can be understood in a more general framework of Bayesian inference.
In \cite{Ghahramani1994}, a joint density model is learned which assigns a likelihood to pairs $(x, y)$.
Probabilistic programming languages aim to execute samples from distributions described by a program, which are conditioned, i.e. restricted by some predicate.
This is equivalent to inverting the probabilistic program and running backwards from observations to causes.
An alternative black-box approach is to not explicitly learn an inverse function at all.
This avoids the non-convexity problem of learning an inverse-mapping from data \cite{jordan1992forward}, but requires an expensive inference procedure for each example.
The advantage of inverse functions is that new elements can be inverted rapidly.
Explicit model inversion for probabilistic inference was demonstrated by stochastic inverses introduced in \cite{Stuhlmueller2013}.
Stochastic inverses invert graphical models by step-by-step execution in reverse order. The term \text{amortized} inference was also introduced to distinguish it as a probabilistic inverse mapping problem, rather than an inverse problem method such as Markov chain Monte Carlo.

\section{Conclusion}

In this contribution we (i) identified a class of problems that benefits from restricting inverse mapping methods to select from a valid preimage (ii) introduced parametric inversion formalism to solve such problems, and (iii) verified our methods by parametrically inverting nontrivial functions.

Three properties emerged as particularly important in parametric inversion: soundness, completeness, and totality.
Our framework could naturally enforce other desired properties, for example interpretability and continuity, by choice of $g$ \todo{\textbf{(is this g the neural net?)}} and regularization of the derivatives of the $f^{-1}$. Other promising future directions include using parametric inversion for variational inference, by imposing a distribution over $\Theta$ rather than optimizing within it.

As previously stated, the number of parameters of a parametric inverse which results from algorithm \ref{algo:compinversion} is a function of the number of primitive functions in the composition.
This will often be far greater than the dimensionality of the preimage of any $y$.

\input{supplementary}

\begin{table*}[h]%\label{tab:pinverses}
  \centering
  \begin{tabular}{ l | c | c | r }
  	$f$ & $R$ & $\Theta$ & $f^{-1}$ \\
    \hline
$x_1+x_2$ & $\mathbb{R}, \mathbb{R}, \mathbb{R}$ & $\mathbb{R}$ & $y = x_1:\mathbb{R} + x_2:\mathbb{R}$ \\
$x_1+x_2$ & $x:\mathbb{R}, \theta:\mathbb{R}$ & $\mathbb{R}$ & $y, z = x + \theta, \theta$ \\
    \hline
  \end{tabular}
\medskip
	  \caption{Primitive parametric inverses.  Column $f$ contains forward non-injective functions. The input space for the forward function $f$ is $X$ while $\Theta$ is the parameter space used for parametric inverses shown in column $f^{-1}$. $\select{a,b}{c}$ denotes if $c$ then $a$ else $b$, or $ac + b(1-c)$}\label{tab:inverses}
\end{table*}

% \section{Glossary}
% \begin{itemize}
% \item $f: X \to Y$ forward function
% \item $f^{-1}: Y \times \Theta \to X$ its parametric inverse
% \item $\Theta$ parameter space of $f^{-1}$
% \item $h: Y \to X$ right inverse of $f$
% \item $h^*$ optimal right inverse
% \item $g: Y \times W \to \Theta$ - parameterized function (neural network) which will select parameters for $f^{-1}$
% \item $W$ Parameter space (weight matrix) of $g$
% \item $\bm{w} \in W$ element of $W$
% \item $f^{-1}_W(y; \bm{w}) = f^{-1}(y; g(y; \theta))$ - parametric inverse reparameterized onto $W$
% \item $\apinv{f}$ Totalized $f^{-1}$
% \item $\mathcal{L}_\circ$ composite loss
% \end{itemize}




==> discussion.tex <==
\section{Discussion}

The primary contributions of this paper are the formalizations of two higher-order probabilistic objects -- the random conditional distribution and the random interventional distribution -- and the probabilistic programming language \omegalang{} which incorporates these objects as primitive constructs.

% % \paragraph{Expressiveness}
% Random conditional distributions increase the expressiveness of probabilistic programming because they allow you to condition on distributional properties.
% In sampling based probabilistic programming languages, a probability distribution is represented as a procedure that generates samples from the distribution.
% This is done by defining a set of primitive samplers, and methods to define procedures which compose them.
% Universal languages such as Church and WebPPL support samplers which return samplers, which are a representation of a random distribution.
% Hence, random conditional distributions and random interventional distributions can be represented in these languages, at least in a model specific way.

% The generic random conditional operator $\parallel$ would require extensions to these languages to implement.
% This is because if a sampler $X$ samples from another sampler $T$, there is no generic mechanism to fix the value $T$ within $X$.
% In \omegalang{}, we achieve this through tracking and manipulation of identifiers, but it is difficult in the standard semantics of sampling based languages.
% In the following example in WebPPL, we cannot construct a sampler for $\rcdxy{X}{T}$ in
%  \texttt{rcdXT}, because there is no mechanism to enforce \texttt{where T() = tsample}, the application \texttt{T()} within \texttt{X} is inaccessible from \texttt{rcdXT}.
% \begin{figure}[h]
%   \centering
%   \begin{BVerbatim}
% var T = function() { return flip() }

% var X = function() { return normal(T(), 1)}

% var function rcdXT = function() {
%   tsample = T()
%   return X // where T() = tsample in X
% \end{BVerbatim}
% \end{figure}

% The consequence of this is that random conditional distributions must be explicitly constructed.
% This is cumbersome, and not in line with the principles discussed in section \ref{higher}, which is that the original model specifies sufficient information to construct all random conditional distributions.
% We achieve this in \omegalang{} through careful tracking and manipulation of identifiers, as described in the operational semantics.


% \paragraph{Inference}
% Conditioning on distributional properties is hard computationally because distributional properties are often expensive or even intractable to compute.
% For instance the KL-divergence between two distributions can be computed in closed form for only a handful of special cases, such as multivariate Gaussians, and approximated from samples  \cite{PrezCruz2008KullbackLeiblerDE} only in low dimensions.


\paragraph{Measure Zero} The random conditional distribution is a distribution over random variables conditioned on measure zero events of the form $\Theta = \theta$.
Conditioning on measure zero events is both routine and problematic, and several approaches have been taken to resolve it.
In his axiomatization of probability, Kolmogorov used not conditional distributions but only conditional expectations.
An alternative approach is in disintegration \cite{chang1997conditioning}, which is less general.  Recent work in \cite{kozen2018disintegration} weakened took a category-theoretic approach to weaken assumptions governing disintegration.
The probabilistic programming language Hakaru \cite{narayanan2016probabilistic} is based on disintegration, and uses equational reasoning to perform exact Bayesian inference on measure zero events.
In future work we intend encode random conditional distributions in these alternative formalisms.

% \paragraph{Future Work}


==> graph.tex <==
\section{Higher Order Graphical Model}{\label{graphical}}

Probabilistic inference means to construct and condition random variables.
In measure theory, a random variable is a function from a sample space $\Omega$ to $T$, where $T$ could for example be $\mathbb{R}$, but any type in general.
$\Omega$ is understood as the universe of possible scenarios that could occur, or in sampling terms, as the random inputs to a random variable.
Measure theory formalizes uncertainty by assigning probabilities to sets of possible scenarios, called events.
The measure of an event represents a degree of belief that the event could occur, and is determined by a probability measure $\mu:\Sigma \rightarrow [0,1]$ where $\Sigma$ is a sigma-algebra (measurable subsets of $\Omega$).
An event $A$ is impossible if $\mu(A)=0$, and certain if $\mu(A)=1$.

We formulate $\rcd$ with respect to a form of directed graphical model.
Higher order directed graphics are similar to standard bayesian networks but depart from them in two significant ways.
First, the semantics of a graph is defined in terms of measure theoretic random variables, in contrast to probability mass or density functions, which means that every node is a deterministic transformation and all randomness is considered external to the system.
Second this graph formalism is based on measure theoretic probability.

\begin{definition}
A higher order Bayesian Network $\mathcal{G}(V,E)$ is a directed acyclic graph, where $V$ are the nodes and $E$ are the edges of the graph.
Nodes correspond to random variables, measurable functions from a sample space $\Omega$ to some output type $T$.
Let $V_{\omega} \subseteq V$ denote the subset of variables without parents.
Higher order graph are able to express both functions between between variables and functions of variables.
Standard (non higher order) models are expressed using edges in $E_\circ$ (read $E$ compose).
A composition edge from $A$ to $B$ denotes that $B$ functionally (and causally) depends on $A$.
More precisely $A \to B$ denotes the composition $B \circ A$.
Since $A$ is random variable, this composition is a random variable $\omega \mapsto B(A(\omega))$.
\end{definition}
Application edges in $E_{apply}$ denote function application.
If a node $A$ is at the source of a directed edge in $E_{apply}$ it is taken as a value to be given as input to the node at the tail.
% Let $f : V \to what$ map each node to a corresponding function, and $id : V_{\omega} \to \mathbb{N}$ map each parent-free node to a unique integer.
  

\begin{align*}
\mu &= \mathcal{N}(0, 1) \\
X &= \mathcal{N}(\mu, 1) \\
\tilde{X} &= \mathbb{E}(\rcdxy{X}{Y})
\end{align*}


==> implement.tex <==
\section{Implementation}\label{implement}
In this section we detail two implementation choices.

\subsection{Memoization of Random Variables}
It is common to have multiple random variables depend on (i.e. are functions of) a shared parent.
This means that in the evaluation of the children, the parent will be evaluated several times on the same input.
If the parent is expensive to compute, this can incur significant unnecessary run-time expense.

We use memoization as a simple counter-measure.
We equip each random variable with a store.
On the first application $x = X(\omega)$ is evaluated as standard but $x$ is stored.
On subsequent applications $x$ is retrieved from the store, rather than recomputed.

Other probabilistic systems such as \cite{le2016inference} have implemented similar mechanisms for similar reasons.
When performing inference in the approach presented by \cite{milch2005, wingate2011lightweight} often a probabilistic program is executed several where on a small number of random variables change between executions.
Caching intermediate results can have large run-time savings.
The same effect could be implemented in \omegalang{} with a more fine grained memoization, which memoizes not just on the equivalence of $\omega$, but on particular components. 


==> motivating.tex <==
\section{Motivating Example}
Our approach is in firm agreement with the semantics of de Finetti, Pearl, and Kyburg, but several problems remain. 
Here, we demonstrate these problems by extending an example from \cite{pearl1987we}, and demonstrate how to use random conditional distributions to construct and condition higher-order probabilities.

In this example there are two coins, $coin_1$ being a typical off-the-street coin, while $coin_2$ is minted in the basement of an notoriously unscrupulous gambler.
The event $E_i$ denotes "the event that $coin_i$ turned up heads".
In Pearl's terms, being unsure about the probability $\prob(E_i)$ means that "one is aware of a set of contingencies", which if true would substantially alter the assessment of the probability of the outcome of $E_i$.
$coin_1$ can be modeled as a Bernoulli distributional in our language \omegalang{} which takes value $1$ when the coin lands heads and has no contingencies:
\begin{figure}[h]
	\centering
	\begin{BVerbatim}
let coin1 = Bernoulli(0.5)
\end{BVerbatim}
\end{figure}

In contrast, $E_2$ has several contingencies since $coin_2$ has a more complex causal structure.
The coin is either fair, biased towards heads (weight 0.6) or biased towards tails (weight 0.4); the probabilities of each scenario are respectively 0.8, 0.1, 0.1.
As a program in \omegalang{}:

\begin{figure}[h]
	\centering
	\begin{BVerbatim}
let coin2 = 
  let isfair = Bernoulli(0.8)
      isbiasedH =  Bernoulli(0.5)
      weight = if isfair then 0.5
               else if isbiasedH then 0.6 else 0.4
        in Bernoulli(weight) 
\end{BVerbatim}
\end{figure}
The marginal probabilities of $E_1$ and $E_2$ are both equal to 0.5, and can be computed in \omegalang{} using \texttt{prob}.
We use the notation \texttt{e => v} to denote that an expression \texttt{e} evaluates to a value \texttt{v}:
\begin{figure}[h]
	\centering
	\begin{BVerbatim}
prob(coin1) => 0.5       prob(coin2) => 0.5
\end{BVerbatim}
\end{figure}

However, these marginal probabilities do not capture the full picture.
Most people would feel much more uncertain about the assessment $\prob(coin_2) = 0.5$ than $\prob(coin_1) = 0.5$.
This is because the former has several contingencies which if true would alter this probability.
The expression \texttt{prob(prob(coin2) = 0.5)} is unfortunately not well typed, since the inner term \texttt{prob(coin2) = 0.5} evaluates to a Boolean, on which $\prob$ has no meaningful definition.
Moreover, we have not specified with respect to which contingencies we would like to consider the uncertainty over \texttt{prob(coin2)}.
In \omegalang{}, the operator $\parallel$ constructs a random conditional distribution over coins:

\begin{figure}[h]
	\centering
  \begin{BVerbatim}
let coin2rcd = coin2 || (isfair, isbiasedH)
\end{BVerbatim}
\end{figure}

Probabilities over probabilities are induced from applying \texttt{prob} to \texttt{coin2rcd}.
That is, while the standard \texttt{prob} maps a Boolean valued random variable to a probability, when applied to a Boolean valued random distribution it yields a distribution over probabilities.

\begin{figure}[h!]
	\centering
  \begin{BVerbatim}
let probdist = prob(coin2rcd) in rand(probdist)
\end{BVerbatim}
\end{figure}

Figure~\ref{probdist1} shows samples of \texttt{prob(coin2rcd)} which are obtained by applying \texttt{rand} to it.

%\begin{figure}[!htb]
%  \centering
%  \includegraphics[width=0.3\linewidth]{coindist}
%  \caption{Distribution over probabilities that $coin2$ comes up heads}
%  \label{probdist1}
%\end{figure}
%  

\begin{figure}[!htb]
  \centering
  \includegraphics[width=0.3\linewidth, trim={.75cm 1cm .8cm 0.95cm},clip]{coindist1}
  %\fbox{\includegraphics[width=0.3\linewidth, trim={.75cm 1cm .8cm 0.95cm},clip]{coindist1}}
  \caption{Distribution over probabilities that $coin2$ comes up heads}
  \label{probdist1}
\end{figure}
  
%\begin{figure}[!htb]
%  \centering
%  %\includegraphics[width=0.3\linewidth, trim={.9cm .55cm 1.1cm 0.95cm},clip]{coindist2}
%  \fbox{\includegraphics[width=0.3\linewidth, trim={.8cm 1cm .8cm .7cm},clip]{coindist2}}
%  \caption{Distribution over probabilities that $coin2$ comes up heads}
%  \label{probdist1}
%\end{figure}
  
By specifying a causal model (a probabilistic program) for predicting the outcome of each event, we have automatically specified the variance in that prediction.
In other words, by specifying the model in terms of causal probabilistic relationships, we automatically specify not only the marginal distributions of variables, but also an entire set of future scenarios, describing how the probabilities would vary in an entire set of scenarios, while also specifying the likelihood of those scenarios.

==> rid.tex <==
\section{The Random Interventional Distribution}\label{rid}

% WTP: dist props with rcd require infernece
Since realizations of random conditional distributions are conditional random variables, simply sampling a distributional property, let alone conditioning it, requires inference.
However, not all problems of conditional inference are equally hard.  As an example, in the model $\Theta = \bern(0.5)$, $X = \normal(\Theta, 1)$, to sample from $\conds{\Theta}{X = 1}$ is more challenging than from than $\conds{X}{\Theta = 1}$.
The former is a Bayesian inference problem whereas in the latter we may simply set $\Theta$ to 1.
This disparity does not arise from distributional differences between $X$ and $\Theta$.
Rather, it is a consequence of causal structure of the model.
%
% Following this intuition, we introduce the random interventional distribution (rid): a distribution over random variables that have been \emph{intervened}, rather than conditioned.
% In a rid, we fix a random variable to a given value as opposed to conditioning on it in a random conditional distribution (rcd).
% As a result, it is cheaper to evaluate a rid than the corresponding rcd.
% In this section, we first introduce what it means to fix the value of a variable, then define the random interventional distribution,
% and finally state when it is correct to replace a rcd with a rid.

% However, in most use cases of a random conditional distribution $\rcdxy{X}{\Theta}$, $\Theta$ is the cause of $X$, i.e., $X$ depends on $\Theta$ rather than the other way around.

% Under modest causal conditions (theorem \ref{thm:rcdrid}) it is permissible to use a different distribution which is more efficient to compute:  $\ridxy{X}{\Theta}$ which \emph{fixes} rather than conditions $\Theta$.

\subsection{Causal Interventions}

Fixing a random variable can be formalized as a causal intervention.
% Difference between intervention and conditioning
Intervention is similar to, but differs from conditioning.
Intervening a random variable only affects the random variables that depend on it (its descendants),
whereas conditioning affects also those variables it depends on (its ancestors).
For instance, to intervene a thermometer such that it reads 80 degrees means to tamper with the thermometer, and does not influence our belief about the weather outside.
Conditioning the thermometer to read 80 degrees, in contrast, makes it more likely that the sun is up.

% Intervention formalized as do opreation
Interventions have been formalized on causal graphical models using the $\doo$ operator.
$\doo(\Theta = \theta_c)$ means that $\Theta$ is fixed to expression $\theta_c$ and effectively cuts edges incoming to $\Theta$, which in the unintervened model determine its value.

$\conds{X}{\doo(\Theta = \theta_c)}$ is a random variable identical to $X$ with the exception that is defined on a model where $\Theta$ is fixed to $\theta_c$.
The implementation is straightforward.
To evaluate $(\conds{X}{\doo(\Theta = \theta_c)})(\omega)$, we first log the variable id of $\Theta$.
Then, when evaluating $X(\omega)$, we intercept any evaluations of $\Theta(\omega)$ (identified by its id), and instead return $\theta_c$

\subsection{Random Interventional Distribution}

Given two random variables $X$ and $\Theta$, the random interventional distribution of $X$ given $\Theta$ -- which we denote $\ridxy{X}{\Theta}$ -- is a a random distribution.
In particular, each realization of $\ridxy{X}{\Theta}$ is the random variable $X$ subject to the intervention $\Theta = \theta$ where $\theta \sim \Theta$ is a realization of $\Theta$:

\begin{definition}The random interventional distribution of a random variable $X: \Omega \to \tau_1$ given $\Theta: \Omega \to \tau_2$ is a random variable $\ridxy{X}{\Theta}: \Omega \to (\Omega \to \tau_1)$, defined as:
\begin{equation}\label{eq:rid}
(\ridxy{X}{\Theta})(\omega) = \conds{X}{\doo(\Theta = \Theta(\omega))}
\end{equation}
\end{definition}

\subsection{Equivalence of rid and rcd}

In general it is more challenging to condition a random variable rather than intervene it.
Naturally, in scenarios when they are equivalent, it is preferable to use the  use $\ridxy{X}{\Theta}$ as a substitute for $\rcdxy{X}{\Theta}$.  
However, in some models $\ridxy{X}{\Theta}$ differs from $\rcdxy{X}{\Theta}$, e.g.:
{\small
\begin{align*}
\alpha &= \unif(\{-1, 1\}) \\
\beta &= \bern(0.5) * \alpha \\
\gamma &= \bern(0.5) + \alpha + \beta
\end{align*}
}
Here, $\rcdxy{\gamma}{\beta} \neq \ridxy{\gamma}{\beta}$.
The distributions over expectations $\ee(\rcdxy{\gamma}{\beta})$ and $\ee(\ridxy{\gamma}{\beta})$ do not even have the same support.
In contrast, $\rcdxy{\gamma}{\alpha}$ is equivalent to  $\ridxy{\gamma}{\alpha}$.

In the case of $\gamma$ and $\beta$, conditioning $\beta$ affects the distribution of $\alpha$ which is used directly in evaluating $\gamma$.
In contrast, intervening $\beta$ has no effect on $\alpha$, and hence intervention and conditioning are not interchangeable.
%
In the case of $\gamma$  and $\alpha$, conditioning $\alpha$ would also affect its ancestors.
%
However, those variables cannot affect the distribution of $\gamma$ without going through $\alpha$.
%
As a result, $\rcdxy{\gamma}{\alpha}$ is equivalent to  $
\ridxy{\gamma}{\alpha}$.

In general, verifying equivalence of two random variables (let alone two random distributions) is undecidable.
%
However, following the above intuition allows us to provide a sufficient condition to determine whether $\ridxy{X}{\Theta} = \rcdxy{X}{\Theta}$.
%
Intuitively, $\ridxy{X}{\Theta} = \rcdxy{X}{\Theta}$ when the ancestors of $\Theta$ can only affect $X$ through $\Theta$.

To formalize this intuition, we first define the parent-child relation between random variables.

\begin{definition}[Parent-Child Dependence] In an execution, a random variable $\Theta$ is a parent of a random variable $X$ iff:
    \begin{enumerate}
        \item When evaluating $X(\omega)$, we need to evaluate $\Theta(\omega)$.
        \item The result of $\Theta(\omega)$ is directly used in evaluating $X(\omega)$ without going through another random variable. More formally, in the derivation tree of the operational semantics, there exists a path between evaluating $\Theta(\omega)$ ($\omega app $ rule) and evaluating $X(\omega)$ such that no other random variable is evaluated.
    \end{enumerate} 
\end{definition}

For example, in the previous program, both $\alpha$ and $\beta$ are parents of $\gamma$.
However, $\alpha$ will not be a parent of $\gamma$ if we define $\gamma$ as $\gamma = \bern(0.5) + \beta$

Following this definition, we can define an acyclic dependence graph $(G,V)$ for each execution, where each vertex $v\in V$ is a random variable, and
each edge $e\in E$ represents a parent-child dependence.
%
We say $v_1$ is an ancestor of $v_2$ if there exists a path from $v_1$ to $v_2$ in the dependence graph.
%
We use $\ance(v)$ to denote all the ancestors of $v$ in an execution.
%
Now, we state formally when rcds and rids are equivalent:

% Given the ancestral relation between variables, we can construct a causal graph from an \omegalang{} program.
% Let $G = (V, E)$ be a directed graph, where $V$ is a set of random variables and $E$ is a set of directed edges which encode causal relations.
% Each edge $e \in E$ is a pair of random variables $(v_1, v_2)$
% There is an edge in $E$ if 

% A path $p = (e_1, ..., e_n)$ is a sequence of edges, where $head(p) := head(e_1)$ and $tail(p) = tail(e_n)$ and for all consequence edge pairs $e_i, e_{i+1}$, $tail(e_i) = head(e_{i+1})$.


% \todo{Maybe use d-separation. $\Theta$ d-separates $X$ from its ancestors}
\begin{theorem}[Rcd and Rid Equivalence Condition]
\label{thm:rcdrid}
For a given execution, $\rcdxy{X}{\Theta} = \ridxy{X}{\Theta}$ if for any $v \in \ance(\Theta) \cap \ance(X)$, $\Theta$ is on all paths between $v$ and $X$.  
\end{theorem}
\begin{proof}
Based on the assumption, for any $v \in \ance(\Theta) \cap \ance(X)$, conditioned on $\Theta$,  $X$ is independent from $v$, i.e.
\begin{equation*}
\conds{X}{\Theta, v} = \conds{X}{\Theta} \quad \text{for all } v \in \ance(\Theta) \cap \ance(X)
\end{equation*}
which implies
\begin{equation*}
    \conds{X}{\Theta, v_1,...,v_n} = \conds{X}{\Theta} 
\end{equation*}
where $\{v_1,...,v_n\} = \ance(\Theta) \cap \ance(X)$.
Therefore, using \eqref{eq:rid} we obtain the following identity for all $\omega$
\begin{align*}
(\ridxy{X}{\Theta})(\omega) &= (\conds{X}{\Theta = \Theta(\omega), v_1 = v_1(\omega),..., v_n = v_n(\omega)}) \\
&= (\conds{X}{\Theta = \Theta(\omega)})
\end{align*}
which concludes the proof that $\rcdxy{X}{\Theta} = \ridxy{X}{\Theta}$.
\end{proof}

Note the dependence graph may vary across executions.
%
Thus, to safely replace a rcd operator with rid operator statically,
one needs to ensure that they are equivalent for all executions.
%
While in principle it is possible to implement a static analysis
to automate the process, we currently rely on the programmer
to perform the replacement manually.

% As a result, there are two ways to exploit opportunities to substitute rcds with rids: dynamic or static.
% %
% In the dynamic approach, the runtime needs to maintain a dependence graph on the fly and check the equivalence
% condition, applies the substitutions dynamically.
% %
% In the static approach, one needs to calculate a dependence graph that overapproximates the dependence graphs of
% all executions and does the substitutions accordingly.
% %
% While it is possible, we have not implemented these methods in \omegalang{}.
% %
% The user can manually replace rcds with rids when they deem these two operators are equivalent on all executions.

==> soundness.tex <==
\subsection{Soundness}

In this section we prove key theorems that the operational semantics respects the denotational semantics
\\
First let us denote a mapping $\textrm{smap}$ from the operational domain to the denotational domain.  $\textrm{smap}(\crvv{f}{i}) = (X, \mathcal{S}', I)$, where $I = \{\textrm{pair}(i, j) \mid j \in \mathbb{N}\}$.  $\textrm{pair}$ is a bijective pairing function mapping two natural numbers to an integer. $\mathcal{S}' = \mathcal{S} \cap \{\omega \mid f(\omega) \neq \bot\}$.
$\textrm{smap}((\omega, i)) = (\omega, I)$ where $I = \{\textrm{pair}(i, j) \mid j \in \mathbb{N}\}$


\begin{theorem}$t_1 \mapsto \crvv{f}{i}$ and $t_2 \mapsto \crvv{g}{j}$ if and only if $I \cap J = \emptyset$ where $I = \sem{t_1}$ and $J = \sem{t_2}$
\end{theorem}
\textit{proof}


\begin{theorem}$t_1 \mapsto \crvv{f}{i}$ and $\ciid(t_2) \mapsto \crvv{f}{j}$ implies $\sem{\ciid(t_2)} \in \ciidset{\sem{t_1}}{\alpha(X)}$.
\end{theorem}
\textit{proof}

\begin{theorem}Let $\sem{t_1} = (X, \mathcal{S}', I)$ where $\mathcal{S}' = (\Omega', \mathcal{H}', \mathcal{P}')$.  $t_1(t_2) \mapsto \bot$ if and only if $\sem{t_2} \in \Omega$ 
\end{theorem}
\textit{proof}

% \begin{theorem}$t \mapsto f$, $\rv(t) \mapsto v$, implies $v \in \ciidset{X}{\alpha(X)}$ where $X = (\sem{t}, \mathcal{S} \cap \{\omega \mid \sem{t}(\omega) \neq \bot \})$
% \end{theorem}
% \textit{proof}

% \begin{theorem}Let $\rv{t} \mapsto v$ implies $v \in \ciidset{X}{\alpha{X}}$ where $X = ()$
% \end{theorem}
% \textit{proof}


